Visual Representations inside the Language Model

Despite interpretability work analyzing VIT encoders and transformer activations, we don't yet understand why Multimodal Language Models (MLMs) struggle on perception-heavy tasks. We offer an under-studied perspective by examining how popular MLMs (LLaVA-OneVision, Qwen2.5-VL, and Llama-3-LLaVA-NeXT) process their visual key-value tokens. We first study the flow of visual information through the language model, finding that image value tokens encode sufficient information to perform several perception-heavy tasks zero-shot: segmentation, semantic correspondence, temporal correspondence, and referring expression detection. We find that while the language model does augment the visual information received from the projection of input visual encodings-which we reveal correlates with overall MLM perception capability-it contains less visual information on several tasks than the equivalent visual encoder (SigLIP) that has not undergone MLM finetuning. Further, we find that the visual information corresponding to input-agnostic image key tokens in later layers of language models contains artifacts which reduce perception capability of the overall MLM. Next, we discuss controlling visual information in the language model, showing that adding a text prefix to the image input improves perception capabilities of visual representations. Finally, we reveal that if language models were able to better control their visual information, their perception would significantly improve; e.g., in 33.3% of Art Style questions in the BLINK benchmark, perception information present in the language model is not surfaced to the output! Our findings reveal insights into the role of key-value tokens in multimodal systems, paving the way for deeper mechanistic interpretability of MLMs and suggesting new directions for training their visual encoder and language model components.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> old_tables/clip_dino_results.tex <==
\begin{table}[t]
% \begin{wraptable}{r}{0.55\linewidth}
\footnotesize
\centering
    \begin{tabular}{lcccc}
    \toprule
        Visual rep.& SPair-71K & \multicolumn{3}{c}{DAVIS}\\
        & PCK & $\mathcal{J}\text{\&}\mathcal{F}_m$ & $\mathcal{J}_m$ & $\mathcal{F}_m$  \\
        \midrule
        CLIP  & 41.4  & 62.5 & 60.6 & 64.4 \\
        DINO  & 36.7 & \textbf{71.4} & \textbf{67.9} & \textbf{74.9} \\  
        \midrule
        LLAVA-OV 7B & \textbf{46.1}  & 65.8 & 62.6 & 67.2 \\
        (Best Value) & & & & \\
      \bottomrule 
    \end{tabular}
\caption{Results of CLIP, DINO and the best LLAVA-OneVision 7B image value on semantic correspondence (per point mean PCK, $\alpha$bbox = 0.1) and temporal correspondence. The visual representations of LLAVA-OneVision 7B outperform DINO and CLIP on semantic correspondence, and CLIP on temporal correspondence.
}
\label{tab:spair71k}
% \end{wraptable}
\end{table}

==> old_tables/combined_correlation_graph_and_clip_dino_table.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{0.55\textwidth}
    \footnotesize
    \centering
        \begin{tabular}{lcccc}
        \toprule
            Visual rep.& SPair-71K & \multicolumn{3}{c}{DAVIS}\\
            & PCK & $\mathcal{J}\text{\&}\mathcal{F}_m$ & $\mathcal{J}_m$ & $\mathcal{F}_m$  \\
            \midrule
            CLIP  & 41.4  & 62.5 & 60.6 & 64.4 \\
            DINO  & 36.7 & \textbf{71.4} & \textbf{67.9} & \textbf{74.9} \\  
            \midrule
            LLAVA-OV 7B & \textbf{46.1}  & 65.8 & 62.6 & 67.2 \\
            (Best Value) & & & & \\
          \bottomrule 
        \end{tabular}
    \captionof{table}{Results of CLIP, DINO and the best LLAVA-OneVision 7B image value on semantic correspondence (per point mean PCK, $\alpha$bbox = 0.1) and temporal correspondence. Intermediate visual representations of LLAVA-OneVision 7B outperform DINO and CLIP on semantic correspondence, and CLIP on temporal correspondence (Sec. \ref{sec:values-clip}).
    }
    \label{tab:clip_dino}
    \end{minipage}
    \hspace{0.02\textwidth}
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/segmentation_vs_downstream.pdf} % Replace with your image file
        \caption{Best-value average segmentation correlates with downstream perception performance (Sec. \ref{sec:downstream_correlation}).}
        \vspace{-1.2cm}
        \label{fig:downstream_correlation}
    \end{minipage}%
\end{figure}

==> old_tables/combined_segmentation_prefixing.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{0.4\textwidth}
    % \footnotesize
    \centering
        \addtolength{\tabcolsep}{-0.3em}
        \begin{tabular}{lc}
        \toprule
            Visual representation& Avg. Segm.\\
            \midrule
            Llama3-LLaVA1.6 8B & 47.5 \\ 
            LLaVA-OV 7B  & 51.8  \\
            Qwen2.5-VL 7B  & \textbf{53.5} \\ 
          \bottomrule 
        \end{tabular}
    \captionof{table}{Average segmentation of the best value per model shows perception capabilities of intermediate visual representations. % across 4 tasks. % Weird metric combination
    }
    \label{tab:segmentation_results}
    \end{minipage}
    \hspace{0.03\textwidth}
    \begin{minipage}{0.54\textwidth}
    \footnotesize
    \centering
        \addtolength{\tabcolsep}{-0.4em}
        \begin{tabular}{lccc}
        \toprule
            & BDD-100K& BDD-100K & RefCOCO\\
            & day+street & night+highway & \\
            \midrule
            No prefixing  & 69.7 & 63.4 & 62.3  \\
            Prefixing  & \textbf{70.4} & \textbf{68.2} & \textbf{64.2} \\  
          \bottomrule 
        \end{tabular}
    \captionof{table}{LLAVA-OneVision 7B best-value segmentation (IOU). Prefixing enables task adaptation, particularly on the challenging ``night+highway'' domain in BDD-100K.
    }
    \label{tab:prefixing_results}
    \end{minipage}
    \vspace{-2em}
\end{figure}

==> sections_v0/0_abstract_v1.tex <==
We don't yet understand why Multimodal Language Models (MLMs) still struggle on perception-heavy tasks, such as semantic segmentation and object localization.
Prior interpretability work focuses largely on analyzing ViT-based encoders or the outputs of transformer blocks.
By contrast, we argue that the key-value (KV) tokens are a critical---and understudied---lens for understanding how MLMs process visual inputs. 
By investigating the visual KV tokens in three popular MLMs (LLAVA-OneVision, Qwen2.5-VL and LLaMA-3-LLaVA-NeXT), we deepen our understanding of how MLMs function and improve outputs.
We first distinguish between input-dependent and input-independent keys and reduce hallucination by 3.2\% in the POPE object identification task by blocking attention to input-independent keys. 
Through probing, we show—for the first time—that value tokens encode sufficient information for many perception-heavy downstream tasks: segmentation, semantic correspondence, temporal correspondence, and referring expression detection. In fact, they outperform strong ViT-based models like CLIP and DINO on purely visual tasks like semantic correspondence and improve when textual prompts precede the image on referring expressions and semantic segmentation, hinting that cross-modality may enrich vision-only applications. 
Surprisingly, although we find that KV segmentation capabilities correlate with downstream MLM perception, in 7.5\% of semantic correspondence instances the MLM fails while KV representations succeed, showing that perception information present in the MLM is not surfaced to the final output.
Our findings pave the way for deeper mechanistic interpretability of MLMs, offering new insights into harnessing KV tokens in multimodal systems.



==> sections_v0/0_abstract_v2.tex <==
We don't yet understand why Multimodal Language Models (MLMs) struggle on perception-heavy tasks.
% , such as semantic segmentation and object localization.
Prior interpretability work focuses largely on analyzing ViT-based encoders or the outputs of transformer blocks.
By contrast, we argue that the key-value (KV) tokens are a critical---and understudied---lens for understanding how MLMs process visual inputs. 
By investigating the visual KV tokens in three popular MLMs (LLAVA-OneVision, Qwen2.5-VL and LLaMA-3-LLaVA-NeXT), we deepen our understanding of how MLMs function and improve outputs.
We first study the flow of visual information through the language model, finding that image value tokens encode sufficient information to perform, zero-shot, several perception-heavy downstream tasks: segmentation, semantic correspondence, temporal correspondence, and referring expression detection. 
% Similar to semantic information in text-only language models, the perception capabilities of the visual representations build slowly in the first 2/3 layers, then falls steeply as the later layers focus on generating the text output.
We find that, while the language model layers do build upon the input visual information received from the projection of input visual encodings, this information has less perception capability than the original vision encoder SigLIP on 3 of 6 tasks we study. 
Next, we discuss the need for better visual representations in the language model, showing that their perception capabilities correlate with better perception of the overall model. We show a promising method to improve perception capabilities of visual representations on three tasks.
Finally, we reveal that language models under-utilize the visual information in their current visual representations, e.g., in 43.6\% of multi-view reasoning instances, perception information present in the language model is not surfaced to the final output!
We conduct an intervention study to identify a reason for the same, finding that input-agnostic image key tokens encode artifacts in later layers of the language model, causing perception capability to suffer.
Our findings pave the way for deeper mechanistic interpretability of MLMs, offering new insights into harnessing KV tokens in multimodal systems.


% We don't yet understand why Multimodal Language Models (MLMs) still struggle on perception-heavy tasks, such as semantic segmentation and object localization.
% Prior interpretability work focuses largely on analyzing ViT-based encoders or the outputs of transformer blocks.
% By contrast, we argue that the key-value (KV) tokens are a critical---and understudied---lens for understanding how MLMs process visual inputs. 
% By investigating the visual KV tokens in three popular MLMs (LLAVA-OneVision, Qwen2.5-VL and LLaMA-3-LLaVA-NeXT), we deepen our understanding of how MLMs function and improve outputs.
% We first distinguish between input-dependent and input-independent keys and reduce hallucination by 3.2\% in the POPE object identification task by blocking attention to input-independent keys. 
% Through probing, we show—for the first time—that value tokens encode sufficient information for many perception-heavy downstream tasks: segmentation, semantic correspondence, temporal correspondence, and referring expression detection. In fact, they outperform strong ViT-based models like CLIP and DINO on purely visual tasks like semantic correspondence and improve when textual prompts precede the image on referring expressions and semantic segmentation, hinting that cross-modality may enrich vision-only applications. 
% Surprisingly, although we find that KV segmentation capabilities correlate with downstream MLM perception, in 7.5\% of semantic correspondence instances the MLM fails while KV representations succeed, showing that perception information present in the MLM is not surfaced to the final output.
% Our findings pave the way for deeper mechanistic interpretability of MLMs, offering new insights into harnessing KV tokens in multimodal systems.



==> sections_v0/1_introduction.tex <==
\section{Introduction}

% P1: set up the question.
Multimodal language models (MLMs) still struggle on perception tasks~\citep{fu2024blink, tong2024eyes}, particularly those that require reasoning over relative depth, object localization, identifying object segments, and spatial understanding~\citep{hu2024visual,ray2024sat,bigverdi2024perception}.
Contemporary studies indicate that such perceptual capabilities can be improved with specialized task-designs or datasets~\citep{ray2024sat,bigverdi2024perception}.
Despite empirical improvements on benchmarks with specialized designs, we lack the scientific tools to dissect what causes these improvements. We conjecture that the answer to this question requires understanding how MLMs represent and reason over visual inputs.


\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/Figure_1.pdf}
    \caption{We study visual representations in the key-value cache within Mutimodal Language Models (MLMs), as they are uninfluenced by text (due to the causal nature of cross-modal attention) and directly contribute to the MLM output. Despite MLMs struggling on perception reasoning \citep{fu2024blink, tong2024eyes}, we find that their intermediate image value tokens encode information for various perception tasks --- calling for further research to surface these capabilities already present within MLMs.}
    \vspace{-2em}
    \label{fig:teaser}
\end{figure*}

% P2: Interpretability can be helpful, but current methods are limited.
Efforts to interpret vision-language models have traditionally focused on two main directions. The first direction analyzes ViT-based encoders such as CLIP~\citep{RadfordKHRGASAM21} and DINO~\citep{caron2021emerging}, aiming to understand how visual features are extracted and mapped into semantic space~\citep{dosovitskiy2020image}. 
For instance, one method identifies the role of each attention head within CLIP, then reduces spurious correlations by removing specific attention heads~\citep{gandelsman2024interpreting}.
The second direction examines the outputs of the transformer blocks that process visual tokens in MLMs \citep{liu2024improved,wang2024qwen2}, e.g.,  finding that visual representations gradually align with textual concepts across layers \citep{neo2024towards}. While insightful, these two directions overlook a critical feature that distinguishes MLMs from traditional ViTs: how visual information is represented and used inside the language module.

% P3: What we do 
We argue that the key-value (KV) tokens corresponding to the visual inputs are a critical—and understudied—lens for understanding how language models process visual information. 
In MLMs, an image is typically encoded by an encoder (with an optional lightweight adapter) and then fed into the LLM as visual tokens. 
Cross-modal attention draws on keys and values to determine what information to retrieve about an image.
Analyzing these KV tokens can clarify how MLMs integrate visual details alongside linguistic context. 
Although interpretability approaches for text-only LLMs have studied the KV-cache \citep{ge2024model}, they focus on improving efficiency and do not translate over when studying visual tokens inside an LLM. 
Moreover, the cache may reveal factors that either enhance or degrade visual fidelity in MLMs, giving us handles to improve perception-oriented tasks.

% Old second half of the intro
% We investigate the internal representations of three popular and distinct models: LLAVA-OneVision \citep{li2025llavaonevision}, Qwen2.5-VL \citep{bai2025qwen25vltechnicalreport}, and LLaMa-3-LLaVa-NeXT \citep{li2025llavanextinterleave}.
% % We find what the visual representations in LLMs encode and how they contribute to the final text generated by the model. 
% We first find that some image key tokens are input-independent, while others are input-dependent. 
% %
% We then probe the image value tokens within the LLM, finding that they encode information sufficient for a variety of perception-heavy downstream tasks: segmentation, semantic correspondence, video object tracking, and referring expression detection. 
% %
% Further, we find that their performance on referring expressions and semantic segmentation improves when a prompt is prefixed to the image, highlighting an advantage of both cross-modality and the promptable nature of KVs.

% We present findings with four major implications. 
% First, we run interventional studies on input-independent image keys at middle-to-later layers of the model, revealing that blocking text queries to these image keys in the attention computation mitigates model hallucination in the POPE object identification task \citep{li-etal-2023-evaluating} by 3.2\% --- leveraging insights from our analyses to improve MLM performance. 
% Second, we find that image value tokens can outperform visual representations from DINO and CLIP on perception tasks such as semantic correspondence --- showing that the cross-modality of visual representations within MLMs can benefit even vision-only tasks. 
% Third, we find that the segmentation capability of MLM image values correlates with the MLMs' performance on several downstream perception-heavy tasks --- showing the importance of high-granularity internal visual representations. 
% Finally, we find that MLMs can fail at perception tasks \textit{despite their visual representations successfully performing the same perception task on the input} --- highlighting the need for mechanistic interpretability work to understand why the capability for perception is present within models but not being surfaced, as well as how to surface the same.

% Our work lays the foundation for further studies in mechanistic interpretability of visual representations in MLMs, as well as how to leverage the same for improved model performance on perception-heavy tasks. 


%%% Scratchpad for Intro Second half (Madeleine)
We investigate the internal KV representations of three popular and distinct models: LLAVA-OneVision 7B \citep{li2025llavaonevision}, Qwen2.5-VL 7B \citep{bai2025qwen25vltechnicalreport}, and LLaMa-3-LLaVa-NeXT 8B \citep{li2025llavanextinterleave}. 
We first find that some image \textit{keys} are input-independent, while others are input-dependent. Using this distinction, we run interventional studies on input-independent image keys in middle-to-later layers of the model, revealing that blocking text queries to these image keys in the attention computation mitigates model hallucination in the POPE object identification task \citep{li-etal-2023-evaluating} by 3.2\%.

We then probe the image \textit{values} within the LLM, finding that they encode information sufficient for a variety of perception-heavy downstream tasks: segmentation, semantic correspondence, temporal correspondence, and referring expression detection. 
These tokens can outperform visual representations from DINO and CLIP on perception tasks such as semantic correspondence.
We further improve their performance on referring expressions and semantic segmentation by prefixing a prompt to the image.
% To tie value tokens' perceptual capabilities with the MLM's overall performance, 
We find that the segmentation capability of MLM image values correlates with the MLM's performance on downstream perception tasks.
However, we also discover that MLMs can fail at perception tasks \textit{despite their visual representations successfully performing the same perception task on the input}. 

These presented findings support five major implications.
First, image values of a MLM exhibit perceptual capabilities. 
Second, the cross-modality of visual representations within MLMs can benefit even vision-only tasks, as image values can outperform CLIP and DINO and incorporate prepended prompts. 
Third, the perceptual capabilities of image values are not always surfaced to the final output, highlighting the need for interpretability work to understand why these capabilities are lost and how they can be retained.
% Third, the perceptual capabilities of image values are not always surfaced to the final output, highlighting the need for mechanistic interpretability work to understand why these capabilities are lost and how they can be retained.
Fourth, the correlation between perception capabilities of image values and MLM outputs supports the importance of high-granularity internal visual representations. 
Finally, investigating the properties of KVs can inform interventions that improve MLM perception. 

Our work lays the foundation for further studies in mechanistic interpretability of visual representations in MLMs, as well as how to leverage the same to improve model performance on perception-heavy tasks --- particularly in the cases we reveal, where the perception capability is already present within the model. 

==> sections_v0/2_related_work.tex <==
\section{Related work}
We discuss three fields of research most relevant to our work.

\noindent\textbf{Multi-modal language models.}
MLMs~\citep{liu2024improved,bai2023qwen} achieve an end-to-end perception-reasoning system by integrating vision encoders~\citep{RadfordKHRGASAM21} into large LLMs~\citep{chiang2023vicuna,Touvron2023Llama2O}, leading to significant breakthroughs in various vision-language tasks such as image captioning~\citep{lin2014microsoft} and visual question answering (VQA)~\citep{hudson2019gqa,goyal2017making}. However, recent studies have pointed out that improvements in VQA tasks often stem from the strong language priors of the language model rather than a precise perception of the input image \citep{fu2024blink, tong2024eyes}. As a result, MLMs perform poorly on vision-centric benchmarks. Most existing studies on perception focus only on the impact of the vision encoder. In contrast, we investigate how the language decoder influences perception. 

\noindent\textbf{Mechanistic interpretability.}
Although optimizing large language models through next-token prediction has led to many emergent behaviors and significant improvements in various language and vision-language tasks, their internal mechanisms remain largely unknown due to their complexity. This lack of understanding also limits our insights into issues like hallucination. Mechanistic interpretability aims to uncover the internal workings of language models, such as information flow, by using tools like the logit lens \citep{interpreting-gpt} and sparse autoencoders (SAEs). However, most existing studies focus on understanding purely language-based models \citep{templeton2024scaling,he2024llama,gao2025scaling}.
Recently, some works have begun exploring the mechanistic interpretability of multimodal language models \citep{liu2025mechanistic}, primarily investigating cross-modal information fusion—specifically, whether the language modality effectively leverages visual information through the attention mechanism \citep{huo2024mmneuron, jiang2024interpreting, zhang2024large}. However, language models not only involve cross-modal fusion but also process visual information further. While a few studies have explored how language models process visual inputs \citep{neo2024towards}, they have not examined the visual representations in the KV cache.
% what is encoded in the final visual representation. 
Our work focuses on understanding the visual representation stored in the language model and how these representations influence the generated language responses.

\noindent\textbf{Visual representation learning.}
Visual representation learning is one of the core problems in computer vision, where a visual encoder transforms raw pixels into a representation that can be applied to various downstream tasks \citep{dosovitskiy2020image}. The quality of this representation is typically evaluated using probing tasks to assess the model's perception capabilities, on tasks such as ImageNet classification \citep{Deng2009ImageNetAl}.  
In MLMs, commonly used visual encoders include CLIP \citep{RadfordKHRGASAM21} and DINO \citep{caron2021emerging}. However, in MLMs, the visual encoder is not the only component that processes visual inputs. The cross-modal decoder that follows the encoder not only handles language tokens but also processes visual tokens. Therefore, it is necessary to use probing tasks to analyze the intermediate visual representations produced by the cross-modal decoder.  
% Unlike other visual representations that encode images as a 2D feature map or a token sequence, the cross-modal decoder represents images in a key-value queryable format.

==> sections_v0/3_preliminary.tex <==
\section{Preliminaries}
% What 3.1 should have:
% Because of autoregressive, you can just cache the whole image and then take in the textual prompt as input and calculate attentions. Async processing: vision and then text. That's why it's important to analyze visual representations THERE, because that's the only place you can disentangle them.
% Representation is a function of the input and weights, where the weights include cross-modality module, but input is only image. So it's a pure vision representation and not cross-modality. 
% Position embedding added to K and Q. 

% What 3.2 should have:
% How it is used to generate the text output

MLMs typically consist of three main components: an image encoder, a lightweight adapter, and a language decoder. The image encoder, often a ViT backbone, processes raw image inputs into a set of embeddings. The connector, usually a linear layer, then projects these embeddings into a space compatible with the language model. Finally, the language decoder, typically a Transformer-based autoregressive model, integrates both textual and visual information to generate responses.
In this section, we discuss how images are processed by the visual encoder, and contrast it with how they are processed by the language model.

\subsection{Image Processing by the Visual Encoder}
Each image is divided into $N$ patches, flattened, and projected into $D$-dimensional embeddings. After adding positional encodings, these embeddings form a sequence: $X = [X_1, X_2, ..., X_N]$,
where $X_i$ is the representation of the $i^\text{th}$ patch.
These patch embeddings are then passed into a Multi-Head Self-Attention mechanism \citep{vaswani2017attention}.

Each patch representation $X_i$ is linearly transformed into three separate vectors: Query ($Q$), Key ($K$), and Value ($V$). This is done using learnable weight matrices:
$Q = XW_Q, K = XW_K, V = XW_V$,
where $W_Q, W_K, W_V$ are learned weight matrices of shape $D \times d_k$ and $Q, K, V$  are of shape $N \times d_k$, where $d_k$ is the dimension of each attention head. 

Self-attention is then computed using the scaled dot-product attention mechanism:
% \vspace{-0.5em}
\[\text{Attention}(Q, K, V) = \text{softmax}\left(\frac{Q(K)^T}{\sqrt{d_k}}\right) V.\]
ViT uses a multi-head attention mechanism in which $h$ self-attention operations, called ``heads'', are run in parallel and concatenated before projection to the output space.
% \[\text{MultiHead}(Q, K, V) = \text{Concat}(\text{head}_1, \text{head}_2, ..., \text{head}_h)W_O\]
Following the attention block, the token representations are passed through a feedforward network (FFN), usually consisting of a two-layer MLP with a nonlinearity between layers. 
Layer normalization and residuals are applied before and after attention and FFN respectively. 
% At the final layer, the representation of the learnable
% ``classification token'' added to the sequence is used to predict the classification task, via an MLP or linear layer. 

Every visual token attends to every other token in a dense global self-attention mechanism. As ViTs compute $Q, K, V$ on the fly for every token in a fully tensorized operation, they do not store representations separately for later querying.


\subsection{Image Processing within the Language Model}
The key differences between image processing in MLMs versus ViT are: (1) an explicit key-value storage mechanism; (2) causal attention; and (3) cross-attention between modalities. We detail each below, along with how they relate to text generation by the language model.

\noindent \textbf{Explicit key-value storage.} In standard transformers, a key-value (KV) cache is used to efficiently store and retrieve token embeddings during self-attention: rather than recomputing attention scores for every token at every step, transformers store keys and values for previously seen tokens. In MLMs, this is operationalized by storing pre-computed visual information as static key-value tokens in the cache, allowing text tokens to selectively retrieve them via causal cross-modal attention.  

\noindent \textbf{Causal attention.} In autoregressive decoding, a causal mask $M$ is applied, preventing tokens from attending to future positions:
\[\text{Attention}(Q, K, V) = \text{softmax}\left(\frac{Q(K)^T}{\sqrt{d_k}} + M\right) V\]
% Here, the mask $M$ ensures that each token can only attend to previous tokens and itself. 
In MLMs, the image is generally positioned before the text in the input. Hence, causal attention ensures that text tokens only attend to previous text and visual tokens, and that visual tokens do not attend to text tokens (i.e., there is one-way querying), allowing them to be pre-computed and stored statically in the KV cache (c.f. Appendix \ref{sec:gqa} for details). 

\noindent \textbf{Cross-modal attention.} Due to the positioning of images before text in the input, the LLM can query visual features when generating text via causal attention, i.e., they can ``look up'' relevant visual information:
$\text{Attention}(Q_\text{text}, K_\text{vision}, V_\text{vision})$.
Vision tokens do not influence text generation directly, i.e., they do not modify the text keys or values (similar to how a text token does not modify successive text tokens in the input).

\noindent \textbf{Text generation by the language  model.} The weighted sum of values omitted by the attention mechanism is passed through the remainder of the transformer block to the next layer, successively until the final layer, when it is normalized, passed through a linear layer and softmax, and generates a prediction probability distribution over the vocabulary, predicting each token of the output auto-regressively. 

% Why we care about values in our probing tasks. 

%In our work, to understand the visual representations within the language model, we study the keys and values in the attention mechanisms corresponding to the image input (c.f. Figure \ref{fig:teaser}). 
%This is for two reasons: firstly, due to the positioning of the image before the text and the use of causal attention, the image keys and values are not influenced by the text input, and serve as a \textbf{purely visual representation};
%and secondly, the visual key-value pairs, once computed, are stored and fixed, allowing text tokens to attend to the keys and retrieve values that \textbf{directly contribute to the output}. Thus, they act as a \textit{proxy for the input image}, remaining accessible throughout any downstream language task.
%Therefore, if we desire stronger perception capabilities from our models, studying what is encoded by the image KVs in the language model is a necessary step.

To understand visual representations within the language model, we study the image-based keys and values in the attention mechanism (c.f. Figure~\ref{fig:teaser}). First, due to causal attention and the typical position of image before text, these key-value pairs are unaffected by the text input and thus form a \textbf{purely visual representation}. Second, once computed, they are stored and fixed, allowing all text tokens to attend to image keys and retrieve values that \textbf{directly contribute to the output}. As such, they serve as a \textit{proxy for the input image}, remaining accessible throughout any downstream language task. Understanding what is encoded in these representations is therefore essential for improving perception in MLLMs.



==> sections_v0/4_keys.tex <==

\section{Image Key Tokens: Can be leveraged to mitigate model hallucination}
% Alternate title: "Input-independent image key tokens in later model layers store artifacts"


\label{sec:keys}
We first study the \textit{keys} corresponding to the image input. We begin by surfacing an understanding of what these keys encode, finding that some of them are input-independent, while others are input-dependent (Sec. \ref{sec:keys-dependent}). We then leverage this understanding to reduce model hallucination on the POPE task \citep{li-etal-2023-evaluating} through an interventional study 
(Sec. \ref{sec:keys-intervention}).

\subsection{What do image key tokens encode?}
\label{sec:keys-dependent}
As keys incorporate positional embeddings, they have an understanding of the spatial context of the image when indexing into the values. We examine the extent to which different keys are influenced by changes to the content of the image.

% Since key tokens incorporate position embeddings, we aim to examine the extent to which different key-value pairs are influenced by positional information.

\noindent\textbf{Experiment.} We randomly sample 1000 images from MSCOCO \citep{lin2014microsoft} and obtain intermediate representations for each of these samples across three models: LLaVA-OneVision 7B \citep{li2025llavaonevision}, Qwen2.5-VL 7B \citep{bai2025qwen25vltechnicalreport} (both of which have four distinct attention heads per layer), and LLaMA-3-LLaVA-NeXT 8B \citep{li2025llavanextinterleave} (which has eight). We then compute the variance of the image key tokens in each head and layer for these models across the 1000 image samples (details in Appendix \ref{sec:key_visualization_section}). 

\noindent\textbf{Results.} Our analysis reveals that key tokens can be categorized into two distinct types based on their variance:  
(1) \textit{Input-independent keys.} These keys have very low (L2$<$200) variance across the input images. 
Most keys in early layers of MLMs are input-independent, and a smaller number of input-independent keys reappear in middle-to-late layers of the language model. 
% typically emerge in earlier layers of the model, although there are some input-independent keys in later layers as well. 
(2) \textit{Input-dependent keys.} These keys have a much higher variance across the input images. They typically dominate in the middle-to-late layers of the model. 

We visualize all image keys of LLaVA-OneVision 7B for two images with a PCA projection in Figure \ref{fig:key_visualization}. Although the two images are very different, the input-independent keys can be seen to remain near-invariant (c.f. Appendix \ref{sec:key_visualization_section} for more visualizations across models).

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/key_visualization.pdf}
    \caption{PCA visualization of all image keys in LLaVA-OneVision 7B for two COCO images. The input-independent image keys (highlighted) alone are nearly constant across images.}
    \label{fig:key_visualization}
    \vspace{-0.5cm}
\end{figure*}

% \noindent \textit{Position-based KV pairs.}  
% These KV pairs are independent of the input image and are primarily determined by positional information. Their key representations remain nearly constant across different images, suggesting that the model utilizes them as a form of fixed spatial prior. Such position-based KV pairs typically emerge in earlier layers or a subset of attention heads in late layers. \todo{Need results for exact numbers?}

% \noindent\textit{Content-based KV pairs.}  
% In contrast, content-based KV pairs are highly dependent on the input image. Their key representations vary significantly across different images, indicating that they capture semantic and object-specific information. Content-based KV pairs dominate from the middle to late layers. \todo{Need results for exact numbers?}

% We visualize the PCA projections of all key visual representations in both models in Fig.~\ref{}\a. The results clearly show that certain key visual representations remain invariant to input, reinforcing the existence of position-based KV pairs.

\subsection{Intervening on input-independent image key tokens in later model layers mitigates hallucination}
% Alternate title: "Input-independent image key tokens in later model layers store artifacts"
\label{sec:keys-intervention}
In ViTs, tokens in middle layers corresponding to background patches tend to encode input-agnostic artifacts rather than useful information about the image, since these regions lack meaningful content \citep{darcet2024vision}.
As discussed in Section \ref{sec:keys-dependent}, we find input-independent keys to dominate in earlier layers of the language model, but, critically, to re-emerge in later layers. We test whether these input-independent keys in middle-to-late layers too, contain input-agnostic artifacts by evaluating on hallucination in object detection. 

% Informed by the re-emergence of input-independent key-value representations in the late layers of the language decoder, a reasonable conjecture is that these input-independent keys are not informative for later tasks. We test whether these input-independent key-value representations contribute to hallucinations in object identification.

\noindent \textbf{Experiment.} 
We conduct experiments with LLaVA-OneVision 7B on the POPE benchmark \citep{li-etal-2023-evaluating}, a dataset with 9,000 test samples designed to evaluate MLM hallucination via object identification. Each question in the benchmark asks whether a specific object exists in the given image. We report F1 score aggregated across all 3 subsets of the benchmark.
%on all three subsets of the benchmark: random, popular and adversarial.

% All image keys in the first four layers of LLaVA-OneVision 7B are input-independent. A smaller number of input-independent keys reappear in the last ten layers. 

Input-independent image keys occur often in early layers, with all keys in the first four layers being input-independent. A smaller number reappears in the last ten layers. 
We conduct an interventional study, blocking text token queries to input-independent image keys in: (1) the first four layers of the model; then (2) the last ten layers of the model.
This method is referred to as ``Attention Knockout'' \citep{geva2023dissecting}.
Notably, we do \textit{not} block text keys that belong to the same attention head as these input-independent image keys, ensuring a focus on understanding the impact of visual representations on model output.

\noindent \textbf{Results.}  
LLaVA-OneVision 7B achieves an F1 score of \textbf{78.1} on POPE. When we intervene on attention to the input-independent keys in the first four layers of the model, performance drops sharply to an F1 score of \textbf{55.4}. However, when we intervene on attention to the input-independent keys in the last ten layers of the model, performance increases to an F1 score of \textbf{81.3}, scoring higher (i.e., hallucinating less) than the original model.

We posit that input-independent image keys in earlier layers play an essential role in aggregating contextual information consistent across different inputs. 
In contrast, middle-to-later layers of the model gradually shift focus toward understanding semantics \citep{neo2024towards}, similar to CNNs \citep{krizhevsky2012imagenet} and pure-text language models \citep{Tenney2019BERTRT}, thus have fewer input-independent keys. 
Hence, the input-independent image keys in middle-to-later layers of the model are likely to encode artifacts, similar to ViTs \citep{darcet2024vision}.  
By removing the influence of these visual representations on the language output, we successfully mitigate MLM hallucinations in object identification.

% \begin{figure*}[]
%     \centering
%     \includegraphics[width=\textwidth]{figures/rough_figure_1b_revised.pdf}
%     \caption{Rough intervention figure. \todo{Cut if space is needed} }
%     \label{fig:teaser}
% \end{figure*}

==> sections_v0/5_values.tex <==
\section{Image Value Tokens: Capable of perception, but not always surfaced}
\label{sec:values}
We next study the \textit{values} corresponding to the image input. These tokens store content used by the model to generate language output, via cross-modal attention. We reveal that value tokens (1) encode sufficient information for many perception tasks (\S~\ref{sec:values-tasks}), (2) can leverage utility from cross-modality on vision-only tasks (\S~\ref{sec:values-prefixing},~\ref{sec:values-clip}), (3) are correlated with downstream performance on perception tasks (\S\ref{sec:values-correlate}). We also highlight how MLMs can be improved given the capabilities of their visual representations (\S\ref{sec:values-mlm}).



\subsection{Image value tokens can perform perception-heavy tasks}
\label{sec:values-tasks}
Individual image values contribute to MLM language generation by aggregating spatially distributed information, per the position encoding added to the corresponding image key. 
Therefore, image values should \textit{encode well-localized semantics} of the image while \textit{maintaining cross-modal alignment}. To assess whether image values satisfy these properties, we probe them on two types of tasks requiring the same: segmentation and correspondence. We discuss each task alongside its experimental setup in greater detail below. Note that all tasks are performed in a \textbf{zero-shot} manner unless otherwise specified.

\noindent\textit{Few-shot foreground segmentation.} We evaluate on Pascal-5i (split 0) \citep{shaban2017one}.
% , which consists of 346 test samples. 
% This is a 5-shot binary segmentation task, where 
We train a linear classifier on top of each image value to perform 5-shot binary segmentation. 

\noindent\textit{Co-segmentation.} We evaluate on MSRC \citep{shotton2006textonboost}, which contains sets of images across which the model must segment a similar object. For each image value, we follow \cite{amir2021deep} and perform spatial clustering to segment objects across images.
% A set of images, which share some similarity (either all of them are animals, or the same object is in both). 
% Take all the images, cluster ---- look at the cited paper.

\noindent\textit{Semantic segmentation.} We evaluate on ImageNet-S \citep{gao2022luss}.
% , a semantic segmentation task on images and classes from ImageNet \citep{krizhevsky2012imagenet}. 
We project the text of the class name into the representational space of the image values using the MLM (independent of the image), then choose the final text token as the representation of the class. We select image values with high dot product with this text token as the segmented region.
% condition on the text of the class name --- same as RefExp

\noindent\textit{Referring expression segmentation.} We evaluate on RefCOCO \citep{kazemzadeh2014referitgame}, which requires grounding language to an object in the image. We follow the same method as semantic segmentation, but with text of the referring expression rather than class name. 
% There's no separate FFN; the model itself projects them into the same space K_text independently. Use the representation of the final token of the text, HxW for image, dot product gives similarity map, set threshold.

\noindent \textit{Semantic correspondence.} We evaluate on SPair71K \citep{min2019spair}, in which models must establish semantic correspondences between keypoints annotated on pairs of images. We find nearest neighbors between images for each image value corresponding to a keypoint.

\noindent \textit{Temporal correspondence.}
We evaluate on DAVIS \citep{pont2017davis}, in which models track keypoints of an object across video frames. We follow the same method as for SPair71K.

\noindent \textbf{Results.} We report the best image value segmentation score for each model, averaged across the four datasets in Table \ref{tab:segmentation_results}, and the best image value correspondence scores for LLaVA-OneVision 7B (representative of our models trained on videos) in Table \ref{tab:clip_dino}. We report image value segmentation scores for individual tasks in Appendix Section \ref{sec:per_task_segmentation}.

We contextualize these results in Sections \ref{sec:values-clip} and \ref{sec:downstream_correlation}, but it is clear that MLM visual representations show the capability to perform a wide variety of perception tasks, from different types of segmentation to different types of correspondence across images.

% First 2 are 28 layers x 4 heads
% LLAMA3: different architecture also with GQA but 32x8 
% Old architectures have 32 heads each, too much.
\vspace{-1em}

\input{tables/combined_segmentation_prefixing}




\subsection{Leveraging the cross-modal and promptable nature of image value tokens for task adaptation}
\label{sec:values-prefixing}

Visual representations in the language model have an interesting capability thanks to their cross-modal nature: 
% Being cross-modal, visual representations in the language model have an advantageous capability: 
they can be made \textit{promptable} by prefixing textual prompts to the visual input. This flexibility allows the model to dynamically adapt its visual representations to better align with specific tasks, in a zero-shot manner.
We study this in the context of two tasks: domain adaptation and referring expression detection. 

\noindent\textbf{Domain adaptation for zero-shot semantic segmentation.} 
We evaluate image values from LLAVA-OneVision 7B on BDD-100K \citep{yu2020bdd100k} under two domains: city street during daytime, and highway during nighttime. We present results in Table \ref{tab:prefixing_results}. By prefixing the image with text specifying the domain (``The image is taken at \{daytime, nighttime\} and it is from \{city street view, highway\}''), performance improves on both domains, but especially the more challenging one. This shows that the visual representations were able to successfully incorporate the text information identifying the domains, then adapt to each.

% \input{tables/clip_dino_results}

\noindent\textbf{Referring expression segmentation.}
We evaluate image values from LLAVA-OneVision 7B on RefCOCO. Without text prefixing, the experiment is as described in Sec. \ref{sec:values-tasks}. As seen in Table \ref{tab:prefixing_results}, when the image caption sourced from COCO captions \citep{chen2015microsoftcococaptionsdata} is prefixed to the image input, the image values achieve modestly improved segmentation results. This shows that the visual representations were able to incorporate the text caption (which contains information about the image, and may contain information about the object to segment) to improve their textual grounding and segmentation capabilities.

Our findings suggest that image values are not only effective for visual understanding, but are also inherently adaptable to linguistic conditioning, enabling more controllable reasoning in both pure-vision (semantic segmentation) and vision-language (textual grounding) tasks.

\input{tables/combined_correlation_graph_and_clip_dino_table}

\subsection{The cross-modal advantage of image value tokens over CLIP and DINO, even on pure-vision tasks}
\label{sec:values-clip}
To further study the advantages of the cross-modal nature of visual representations in the language model, we compare the performance of MLM image values to that of traditional visual representations: CLIP \citep{RadfordKHRGASAM21}\footnote{CLIP visual representations have some cross-modality through the supervision of the dot product with text. However, it is much less compared to those within MLMs, which are first projected into the representational space of the text tokens, then further processed by the language model.} and DINO \citep{caron2021emerging}. 
Visual representations from CLIP and DINO show strong performance on both semantic and temporal correspondence, on SPair71K and DAVIS respectively \citep{tang2023emergent}. In Table \ref{tab:clip_dino}, however, we find that the best image value performance of LLAVA-OneVision 7B is higher than both CLIP and DINO on SPair71K, and higher than CLIP on DAVIS. 

Our results again underscore the advantage of cross-modality, allowing these intermediate visual representations of MLMs to beat pure-vision representations on pure-vision tasks. 

\subsection{Better perception of image values correlates with better perception of the model}
\label{sec:values-correlate}
Having studied the perception capabilities of MLMs' intermediate representations by probing image value tokens for perception tasks such as segmentation (c.f. Section \ref{sec:values-tasks}), we further assess MLMs' end-to-end perception reasoning by evaluating them on the perception-heavy vision-language reasoning tasks CV-Bench \citep{tong2024cambrian} and BLINK \citep{fu2024blink}. 
This allows us to investigate a key question: \textit{Does improved perception of intermediate visual representations correlate with better perception reasoning of the model itself?}

% To evaluate the quality of perception in MLMs, we use the performance of stored visual representations on vision-centric tasks such as segmentation as a measure of MLMs’ \textit{perception capabilities}. We then assess their performance on vision-language tasks to evaluate their influence on \textit{end-to-end perception-reasoning}. 
% This allows us to investigate a key question: \textit{Does improved perception correlate with better perception-reasoning?}

\noindent \textbf{Experiment.} 
% We calculate the perception capabilities of the MLM intermediate visual representations by using the maximum segmentation performance across all image values, averaged across four segmentation benchmarks: Pascal-5i, MSRC, ImageNet-S and RefCOCO (c.f. Section \ref{sec:values-tasks}).
To calculate MLMs' end-to-end perception reasoning capability, we evaluate on two vision-centric VQA benchmarks: CV-Bench and the perception-heavy tasks in BLINK. 
CV-Bench consists of 2,637 test samples and assesses MLMs' 2D and 3D perception capabilities in a single image, covering four major categories: counting, relations, depth estimation, and distance estimation. BLINK, on the other hand, contains multi-image questions as well as single-image. Since certain question types in BLINK, such as art style, are less relevant to perception, we select a subset of BLINK consisting of four perception-related tasks: counting, object localization, relative depth, and spatial relations, totaling 1,021 test samples. We evaluate MLMs across these 3,658 test samples to estimate their perception reasoning ability. We compare this to MLM values' segmentation capabilities averaged across four tasks: Pascal-5i, MSRC, ImageNet-S and RefCOCO (c.f. Section \ref{sec:values-tasks}).

\label{sec:downstream_correlation}

% \begin{wrapfigure}{l}{0.5\textwidth}
% \vspace{-1.5em}
% \includegraphics[width=0.95\linewidth]{figures/segmentation_vs_downstream.pdf} 
% \caption{Segmentation performance of LLAVA-OneVision and QwenVL models versus downstream performance. Segmentation is averaged across four datasets, and downstream performance is averaged across CV-Bench and a subset of BLINK (c.f. Section \ref{sec:downstream_correlation}).} 
% \vspace{-2em}
% \label{fig:downstream_correlation}
% \end{wrapfigure}

We evaluate two MLMs with different configurations: (1) models of the same version but different sizes: LLaVA-OneVision (0.5B, 7B, 72B); and (2) models of the same size but different versions: Qwen2-VL 7B and Qwen2.5-VL 7B.  
The LLaVA-OneVision 0.5B model stores 2 key-value pairs per layer, the 7B model stores 4 key-value pairs per layer, and the 72B model stores 8 key-value pairs per layer.


\noindent \textbf{Results.}  
As shown in Figure \ref{fig:downstream_correlation}, we observe that MLMs of different sizes and versions exhibit the same trend: the stronger the perception capability of their image values, as estimated by their segmentation performance, the better the MLMs themselves perform on downstream perception reasoning vision-language tasks.

This finding shows that improved perception of MLM intermediate visual representations goes hand-in-hand with better perception reasoning capabilities of the model itself on perception-heavy vision-language tasks --- 
showing the importance of high-granularity visual representations, and
further emphasizing the need to study the same in MLMs.

% This finding supports two key conclusions. First, value tokens that better encode well-localized semantics positively contribute to MLMs' performance on vision-language tasks. Second, the challenges in MLMs' end-to-end perception-reasoning partly stem from perception itself—that is, the inability to learn sufficiently good visual representations for downstream language tasks, rather than merely being a vision-language alignment issue.

\subsection{Image value tokens show that our MLMs should be doing better at perception}
\label{sec:values-mlm}

Our motivation to study the intermediate visual representations of MLMs was their poor performance on end-to-end perception reasoning \citep{fu2024blink, tong2024eyes}. How, then, are their image values capable of perception, as we show in Sections \ref{sec:values-tasks}--\ref{sec:values-clip}? 
% We find that, although the visual representations may be capable of perception, this capability does not always propagate through the model to the text output: revealing room for improvement to surface the capabilities already present within MLMs.

\noindent\textbf{Experiment.} Semantic correspondence can be framed as a VQA; it can also be evaluated directly from the visual representations (as in Sec. \ref{sec:values-tasks}).
We posit that the image values being able to perform semantic correspondence on an example is a sufficient 
(if not necessary, in case the language model can compensate with its reasoning capabilities) 
condition for the MLM answering the VQA corresponding to the example correctly.

We first frame semantic correspondence in SPair71K as a VQA task, as in BLINK (for which image coordinates are not public), generating 200 samples. We evaluate the MLM on VQA. We then evaluate its intermediate values on semantic correspondence as an image pair, as in Sec. \ref{sec:values-tasks}. 
% \footnote{As we did not have the image coordinates for semantic correspondence on BLINK, we recreate the VQA task with SPair71K images, following the same method as BLINK (itself sourced from SPair71K).} 
We calculate the fraction of instances where the MLM predicts the VQA answer incorrectly, \textit{despite its image values predicting semantic correspondence correctly for the same input}. 

\noindent\textbf{Results.} The accuracy of LLAVA-OneVision 7B on semantic correspondence VQA is 36\%. On only 2.5\% of these, the intermediate value was incorrect but the MLM prediction was correct, showing the importance of visual representations for this task. However, on 7.5\% of the examples, the MLM predicted incorrectly despite the intermediate values predicting correctly! In other words, if the model had successfully surfaced the perception capability of its visual representations, it would have achieved an accuracy of 43.5\% rather than 36\%.  

% value yes, MLLM yes: 67 --> 33.5
% Only value correct (value yes, MLLM no) : 15 --> 7.5
% Only MLLM correct (value no, MLLM yes) : 5 --> 2.5
% Both incorrect (value no, MLLM no) : 113 --> 56.5

Our finding reconciles the perception capabilities of MLMs' intermediate visual representations with their subpar performance on perception reasoning tasks. More importantly, it reveals the potential of MLMs to achieve better perception: underscoring the need for future work to focus on surfacing the capabilities already present within MLMs.

% \input{tables/segmentation_results}

==> sections_v0/6_discussion.tex <==
\section{Discussion and Future Work}
Our investigation throws light on an as-yet under-explored component of MLMs: the visual representations stored in the key-value cache and attended to during text generation, in contrast to existing work, which has studied the transformer block outputs within MLMs \citep{neo2024towards, zhang2024large}.
We find that: (1) a deeper understanding of what these tokens encode allows us to make interventions to improve the model; (2) image value tokens can perform perception tasks, and their performance goes hand-in-hand with perception reasoning of the MLM itself; (3) cross-modality of the visual representations allows benefits such as promptability for flexible task adaptation, as well as outperforming pure-visual representations even on pure-vision tasks; and (4) the perception capabilities of image value tokens reveal room for improvement in perception reasoning by MLMs.
% , calling for research in surfacing these intermediate visual representations' capabilities in the output of the model itself. 

Our work calls for research in three main directions: first, studying more closely what text is generated when various image keys are attended to or blocked to determine whether fixed image keys have fixed purposes (as suggested by Section \ref{sec:keys}); second, understanding more deeply the benefits of cross-modality on vision and vision-language tasks; and third, surfacing intermediate visual representations' perception capabilities in the output of the model itself.
Our work highlights the importance of interpreting image processing by MLMs by studying visual representations in language models, and show promise for the future of perception reasoning in MLMs.


% Our investigation finds that \textbf{KV tokens help us understand how language models process visualization} and \textbf{show promise for improving performance on perception-heavy tasks overall}. 

% % For space, we could make these just bolded headers rather than subsections
% \paragraph{KV tokens are not a monolith, they encode information we can interpret}
% - We found the input dependent and independent, but are there controlled experiments we could run to see more precisely what the keys and values are doing?     
%     - Something like interpretability work in CLIP (e.g., Interpreting CLIP's Image Representation via Text-Based Decomposition) but for this? 
%     - Comparing across multiple (https://distill.pub/2019/activation-atlas/)
%     - Maybe which are activated more for different classes (https://distill.pub/2021/multimodal-neurons/) 
%     - Can we use interpretability methods to show the impact of prepending? 
%     - Can we see which are attended to more for different tasks? 
%     - Can we use the hierarchical nature more explicitly? 

% \paragraph{Using KV tokens to inform interventions can reduce hallucinations}
% - We did an initial study on later vs earlier layers. Can we be more precise and do more ablations to understand the types of hallucinations impacted here?
% - I think qualitative investigation into the impacts of different interventions here could be interesting, but idk if we want to include that. 
% - Can we leverage the hierarchical nature more explicitly and see if this reduces hallucinations? 

% \paragraph{KV tokens in multi-modal language models can outperform DINO and CLIP on purely visual tasks}
% - How can prepending to impact the way that values work affect the values and how does that affect the output? Or basically how can we push this thread even further for perceptual tasks? Since incorporating text can help, can we see what types of text help the most? 
% - More systematic study of the types of outputs that KV tokens are outperforming on, and why that might be related to language

% \paragraph{KV tokens hold perceptual capabilities that are not currently surfaced to final MLM outputs}
% - Why is this information in the internal representations but not being surfaced? How do we surface it — is it just a question of adding more perception-heavy tasks to finetuning (something that I don’t believe is currently being done much), or do we need something more, and if so, what would that “something more” look like?
% - Could we improve on things like BLINK by surfacing perceptual capabilities that are there but hidden? 
% - How might surfacing these capabilities more explicitly help beyond just perception-heavy tasks? 

% \noindent \textbf{Limitations}

% \noindent \textbf{Conclusion}

==> sections_v1/0_abstract.tex <==


Despite interpretability work analyzing VIT encoders and transformer activations, we don't yet understand why Multimodal Language Models (MLMs) struggle on perception-heavy tasks.
We offer an understudied lens by examining how popular MLMs (LLAVA-OneVision, Qwen2.5-VL, and LLaMA-3-LLaVA-NeXT) process their visual key-value (KV) tokens.
We first study the flow of visual information through the language model, finding that image value tokens encode sufficient information to perform, zero-shot, several perception-heavy downstream tasks: segmentation, semantic correspondence, temporal correspondence, and referring expression detection. 
% Similar to semantic information in text-only language models, the perception capabilities of the visual representations build slowly in the first 2/3 layers, then falls steeply as the later layers focus on generating the text output.
We find that, while the language model layers do augment the input visual information received from the projection of input visual encodings, this information loss \ranjay{I changed this to information loss but idk } results in loss of perception capability than the input tokens from the vision encoder (SigLIP) across 3 of 6 tasks we study \ranjay{weird wording... what happens for the other 3 tasks?}. 
Next, we discuss the need for better visual representations in the language model, showing that their perception capabilities correlate with better perception of the overall model \ranjay{This feels kinda obvious? Is it worth highlighting in the abstract?}. We show a promising method to improve perception capabilities of visual representations on three tasks \ranjay{Vague. What is this method?}.
Finally, we reveal that language models under-utilize the visual information in their current visual representations, e.g., in 43.6\% of multi-view reasoning instances, perception information present in the language model is not surfaced to the final output!
We conduct an intervention study to understand why, finding that input-agnostic image key tokens encode artifacts in later layers of the language model, causing perception capability to suffer.
Our findings pave the way for deeper mechanistic interpretability of MLMs, offering new insights into harnessing KV tokens in multimodal systems.


% We don't yet understand why Multimodal Language Models (MLMs) still struggle on perception-heavy tasks, such as semantic segmentation and object localization.
% Prior interpretability work focuses largely on analyzing ViT-based encoders or the outputs of transformer blocks.
% By contrast, we argue that the key-value (KV) tokens are a critical---and understudied---lens for understanding how MLMs process visual inputs. 
% By investigating the visual KV tokens in three popular MLMs (LLAVA-OneVision, Qwen2.5-VL and LLaMA-3-LLaVA-NeXT), we deepen our understanding of how MLMs function and improve outputs.
% We first distinguish between input-dependent and input-independent keys and reduce hallucination by 3.2\% in the POPE object identification task by blocking attention to input-independent keys. 
% Through probing, we show—for the first time—that value tokens encode sufficient information for many perception-heavy downstream tasks: segmentation, semantic correspondence, temporal correspondence, and referring expression detection. In fact, they outperform strong ViT-based models like CLIP and DINO on purely visual tasks like semantic correspondence and improve when textual prompts precede the image on referring expressions and semantic segmentation, hinting that cross-modality may enrich vision-only applications. 
% Surprisingly, although we find that KV segmentation capabilities correlate with downstream MLM perception, in 7.5\% of semantic correspondence instances the MLM fails while KV representations succeed, showing that perception information present in the MLM is not surfaced to the final output.
% Our findings pave the way for deeper mechanistic interpretability of MLMs, offering new insights into harnessing KV tokens in multimodal systems.



==> sections_v1/1_introduction.tex <==
\section{Introduction}

% P1: set up the question.
Multimodal language models (MLMs) still struggle on perception tasks~\citep{fu2024blink, tong2024eyes}, particularly those that require reasoning over relative depth, object localization, identifying object segments, and spatial understanding~\citep{hu2024visual, kamath-etal-2023-whats}.
Contemporary studies indicate that such perceptual capabilities can be improved with specialized task-designs or datasets~\citep{ray2024sat,bigverdi2024perception}.
Despite empirical improvements on benchmarks with specialized designs, we lack the scientific tools to dissect what causes these improvements. We conjecture that the answer to this question requires understanding how MLMs represent and reason over visual inputs.


\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/Figure_1.pdf}
    \caption{We study visual representations in the key-value cache within Mutimodal Language Models (MLMs), as they are uninfluenced by text (due to the causal nature of cross-modal attention) and directly contribute to the MLM output. Despite MLMs struggling on perception reasoning \citep{fu2024blink, tong2024eyes}, we find that their intermediate image value tokens encode information for various perception tasks zero-shot---calling for further research to surface these capabilities already present within MLMs.}
    \vspace{-2em}
    \label{fig:teaser}
\end{figure*}

% P2: Interpretability can be helpful, but current methods are limited.
Efforts to interpret vision-language models have traditionally focused on two main directions. The first direction analyzes ViT-based encoders such as CLIP~\citep{RadfordKHRGASAM21} and DINO~\citep{caron2021emerging}, aiming to understand how visual features are extracted and mapped into semantic space~\citep{dosovitskiy2020image}. 
For instance, one method identifies the role of each attention head within CLIP, then reduces spurious correlations by removing specific attention heads~\citep{gandelsman2024interpreting}.
The second direction examines the outputs of the transformer blocks that process visual tokens in MLMs \citep{liu2024improved,wang2024qwen2}, e.g.,  finding that visual representations gradually align with textual concepts across layers \citep{neo2024towards}. While insightful, these two directions overlook a critical feature that distinguishes MLMs from traditional ViTs: how visual information is represented and used inside the language model.

% P3: What we do 
We argue that the key-value (KV) tokens corresponding to the visual inputs are a critical—and understudied—lens for understanding how language models process visual information. 
In MLMs, an image is typically encoded by an encoder (with an optional lightweight projection) and then fed into the LLM as visual tokens. 
Cross-modal attention draws on keys and values to determine what information to retrieve about an image.
Analyzing these KV tokens can clarify how MLMs integrate visual details alongside linguistic context. 
Although interpretability approaches for text-only LLMs have studied the KV-cache \citep{ge2024model}, they focus on improving efficiency and do not translate over when studying visual tokens inside an LLM. 
Moreover, the cache may reveal factors that either enhance or degrade visual fidelity in MLMs, giving us handles to improve perception-oriented tasks.

We investigate the internal KV representations of three popular and distinct models: LLAVA-OneVision 7B \citep{li2025llavaonevision}, Qwen2.5-VL 7B \citep{bai2025qwen25vltechnicalreport}, and LLaMa-3-LLaVa-NeXT 8B \citep{li2025llavanextinterleave}. We first study the flow of visual information through the language model, focusing on the image value tokens in different layers. We find that these image value tokens encode sufficient information to perform zero-shot perception-heavy tasks: foreground segmentation, semantic segmentation, co-segmentation, referring expression segmentation, semantic correspondence, and temporal correspondence.
Similar to semantic information in text-only language models, the perception capabilities of the visual representations build slowly in the first 2/3 layers \ranjay{Is this still true? Can you mention what experiment proves this?}, then falls steeply as the later layers focus on generating the text output \ranjay{I don't think you can say that the later layers focus on generating text. What you have evidence for is that they no longer encode sufficient visual information. You \textit{conjecture} that this is because of language generation but you can't say that for sure.}.
However, while the language model layers do initially build upon the input visual information received from the projection of input visual encodings, we find that they have less perception capability \ranjay{Not sure what perception capability of an encoding means. Not defined yet.} than the original vision encoder SigLIP on 3 of 6 tasks we study, revealing the need for different methods to train the visual encoder during multimodal training of VLMs \ranjay{Too vague and feels like a jump in conclusion.}. This agrees with findings from concurrent work \citep{fu2025hidden}.

Next, we discuss the need for better visual representations in the language model \ranjay{why? This sentence needs to be connected to the previous one better.}. We show that the perception capabilities of intermediate visual representations, as measured by their segmentation performance, correlates with performance of the overall VLM on perception-heavy downstream tasks. We show a promising method to improve perception capabilities of visual representations: we leverage the promptable nature of language model representations by adding a textual prefix to the image. We find that this allows the model to dynamically adapt \ranjay{You want to mention that you don't train the model. And you need to explain what dynamically adapt means. Maybe even add a visualization if you can show this qualitatively.} its visual representations based on the prefix, improving their performance on three tasks: referring expression segmentation, semantic correspondence and domain adaptation for zero-shot semantic segmentation. 

\ranjay{I understood only this paragraph completely:} Finally, we study language model utilization of \textit{existing} visual representations. We evaluate VLMs on perception-heavy VQA tasks, and their intermediate visual representations on the equivalent zero-shot perception task. We find that in 33.3\% of art style instances \ranjay{art style instances comes out of nowhere and unexplained.}, the VLM answers the question incorrectly, \textit{despite its visual representations performing the task on that same input correctly}---revealing that language models severely under-utilize the information in their existing visual representations. 
We conduct an intervention study to identify a reason for this, finding that input-agnostic image key tokens encode artifacts in later layers of the language model, causing perception capabilities to suffer. We leverage this finding to improve VLM performance on hallucination and general perception benchmarks.


% Next, we discuss the need for better visual representations in the language model, showing that their perception quality correlates with better perception of the overall model. We show a promising method to improve perception capabilities of visual representations on three tasks.
% Finally, we reveal that language models under-utilize the visual information in their current visual representations, e.g., in 7.5\% of semantic correspondence instances, perception information present in the language model is not surfaced to the final output. 
% We conduct an intervention study to identify a reason for the same, finding that input-agnostic image key tokens encode artifacts in later layers of the language model, causing perception capability to suffer.
% Our findings pave the way for deeper mechanistic interpretability of MLMs, offering new insights into harnessing KV tokens in multimodal systems.


% Old second half:
% We investigate the internal KV representations of three popular and distinct models: LLAVA-OneVision 7B \citep{li2025llavaonevision}, Qwen2.5-VL 7B \citep{bai2025qwen25vltechnicalreport}, and LLaMa-3-LLaVa-NeXT 8B \citep{li2025llavanextinterleave}. 
% We first find that some image \textit{keys} are input-independent, while others are input-dependent. Using this distinction, we run interventional studies on input-independent image keys in middle-to-later layers of the model, revealing that blocking text queries to these image keys in the attention computation mitigates model hallucination in the POPE object identification task \citep{li-etal-2023-evaluating} by 3.2\%.

% We then probe the image \textit{values} within the LLM, finding that they encode information sufficient for a variety of perception-heavy downstream tasks: segmentation, semantic correspondence, temporal correspondence, and referring expression detection. 
% These tokens can outperform visual representations from DINO and CLIP on perception tasks such as semantic correspondence.
% We further improve their performance on referring expressions and semantic segmentation by prefixing a prompt to the image.
% % To tie value tokens' perceptual capabilities with the MLM's overall performance, 
% We find that the segmentation capability of MLM image values correlates with the MLM's performance on downstream perception tasks.
% However, we also discover that MLMs can fail at perception tasks \textit{despite their visual representations successfully performing the same perception task on the input}. 

% These presented findings support five major implications.
% First, image values of a MLM exhibit perceptual capabilities. 
% Second, the cross-modality of visual representations within MLMs can benefit even vision-only tasks, as image values can outperform CLIP and DINO and incorporate prepended prompts. 
% Third, the perceptual capabilities of image values are not always surfaced to the final output, highlighting the need for interpretability work to understand why these capabilities are lost and how they can be retained.
% % Third, the perceptual capabilities of image values are not always surfaced to the final output, highlighting the need for mechanistic interpretability work to understand why these capabilities are lost and how they can be retained.
% Fourth, the correlation between perception capabilities of image values and MLM outputs supports the importance of high-granularity internal visual representations. 
% Finally, investigating the properties of KVs can inform interventions that improve MLM perception. 

Our work lays the foundation for further studies in mechanistic interpretability of visual representations in MLMs, as well as how to leverage the same to improve model performance on perception-heavy tasks --- particularly in the cases we reveal, where the perception capability is already present within the model. 

==> sections_v1/2_related_work.tex <==
\section{Related work}
We discuss three fields of research most relevant to our work.

\noindent\textbf{Multi-modal language models.}
MLMs~\citep{liu2024improved,bai2023qwen} achieve an end-to-end perception-reasoning system by integrating vision encoders~\citep{RadfordKHRGASAM21} into large LLMs~\citep{chiang2023vicuna,Touvron2023Llama2O}, leading to significant breakthroughs in various vision-language tasks such as image captioning~\citep{lin2014microsoft} and visual question answering (VQA)~\citep{hudson2019gqa,goyal2017making}. However, recent studies have pointed out that improvements in VQA tasks often stem from the strong language priors of the language model rather than a precise perception of the input image \citep{fu2024blink, tong2024eyes}. As a result, MLMs perform poorly on vision-centric benchmarks. Most existing studies on perception focus only on the impact of the vision encoder. In contrast, we investigate how the language decoder influences perception. Concurrent to our work, \citet{fu2025hidden} reveal that language models fail to utilize visual information captured by the visual encoder. \amita{Add a little bit here.}

\noindent\textbf{Mechanistic interpretability.}
Although optimizing large language models through next-token prediction has led to many emergent behaviors and significant improvements in various language and vision-language tasks, their internal mechanisms remain largely unknown due to their complexity. This lack of understanding also limits our insights into issues like hallucination. Mechanistic interpretability aims to uncover the internal workings of language models, such as information flow, by using tools like the logit lens \citep{interpreting-gpt} and sparse autoencoders (SAEs). However, most existing studies focus on understanding purely language-based models \citep{templeton2024scaling,he2024llama,gao2025scaling}.
Recently, some works have begun exploring the mechanistic interpretability of multimodal language models \citep{liu2025mechanistic}, primarily investigating cross-modal information fusion—specifically, whether the language modality effectively leverages visual information through the attention mechanism \citep{huo2024mmneuron, jiang2024interpreting, zhang2024large}. However, language models not only involve cross-modal fusion but also process visual information further. While a few studies have explored how language models process visual inputs \citep{neo2024towards}, they have not examined the visual representations in the KV cache.
% what is encoded in the final visual representation. 
Our work focuses on understanding the visual representation stored in the language model and how these representations influence the generated language responses.

\noindent\textbf{Visual representation learning.}
Visual representation learning is one of the core problems in computer vision, where a visual encoder transforms raw pixels into a representation that can be applied to various downstream tasks \citep{dosovitskiy2020image}. The quality of this representation is typically evaluated using probing tasks to assess the model's perception capabilities, on tasks such as ImageNet classification \citep{Deng2009ImageNetAl}.  
In MLMs, commonly used visual encoders include CLIP \citep{RadfordKHRGASAM21} and DINO \citep{caron2021emerging}. However, in MLMs, the visual encoder is not the only component that processes visual inputs. The cross-modal decoder that follows the encoder not only handles language tokens but also processes visual tokens. Therefore, it is necessary to use probing tasks to analyze the intermediate visual representations produced by the cross-modal decoder.  
% Unlike other visual representations that encode images as a 2D feature map or a token sequence, the cross-modal decoder represents images in a key-value queryable format.

==> sections_v1/3_preliminary.tex <==
\section{Preliminaries}
\label{sec:preliminary}
% What 3.1 should have:
% Because of autoregressive, you can just cache the whole image and then take in the textual prompt as input and calculate attentions. Async processing: vision and then text. That's why it's important to analyze visual representations THERE, because that's the only place you can disentangle them.
% Representation is a function of the input and weights, where the weights include cross-modality module, but input is only image. So it's a pure vision representation and not cross-modality. 
% Position embedding added to K and Q. 

% What 3.2 should have:
% How it is used to generate the text output

MLMs typically consist of three main components: an image encoder, a lightweight adapter, and a language decoder. The image encoder, often a ViT backbone, processes raw image inputs into a set of embeddings. The connector, usually a linear layer, then projects these embeddings into a space compatible with the language model. Finally, the language decoder, typically a Transformer-based autoregressive model, integrates both textual and visual information to generate responses.
In this section, we discuss how images are processed by the visual encoder, and contrast it with how they are processed by the language model.

\subsection{Image Processing by the Visual Encoder}
\label{sec:preliminary_ve}
Each image is divided into $N$ patches, flattened, and projected into $D$-dimensional embeddings. After adding positional encodings, these embeddings form a sequence: $X = [X_1, X_2, ..., X_N]$,
where $X_i$ is the representation of the $i^\text{th}$ patch.
These patch embeddings are then passed into a Multi-Head Self-Attention mechanism \citep{vaswani2017attention}.

Each patch representation $X_i$ is linearly transformed into three separate vectors: Query ($Q$), Key ($K$), and Value ($V$). This is done using learnable weight matrices:
$Q = XW_Q, K = XW_K, V = XW_V$,
where $W_Q, W_K, W_V$ are learned weight matrices of shape $D \times d_k$ and $Q, K, V$  are of shape $N \times d_k$, where $d_k$ is the dimension of each attention head. 

Self-attention is then computed using the scaled dot-product attention mechanism:
% \vspace{-0.5em}
\[\text{Attention}(Q, K, V) = \text{softmax}\left(\frac{Q(K)^T}{\sqrt{d_k}}\right) V.\]
ViT uses a multi-head attention mechanism in which $h$ self-attention operations, called ``heads'', are run in parallel and concatenated before projection to the output space.
% \[\text{MultiHead}(Q, K, V) = \text{Concat}(\text{head}_1, \text{head}_2, ..., \text{head}_h)W_O\]
Following the attention block, the token representations are passed through a feedforward network (FFN), usually consisting of a two-layer MLP with a nonlinearity between layers. 
Layer normalization and residuals are applied before and after attention and FFN respectively. 
% At the final layer, the representation of the learnable
% ``classification token'' added to the sequence is used to predict the classification task, via an MLP or linear layer. 

Every visual token attends to every other token in a dense global self-attention mechanism. As ViTs compute $Q, K, V$ on the fly for every token in a fully tensorized operation, they do not store representations separately for later querying.


\subsection{Image Processing within the Language Model}
\label{sec:preliminary_llm}
The key differences between image processing in MLMs versus ViT are: (1) an explicit key-value storage mechanism; (2) causal attention; and (3) cross-attention between modalities. We detail each below, along with how they relate to text generation by the language model.

\noindent \textbf{Explicit key-value storage.} In standard transformers, a key-value (KV) cache is used to efficiently store and retrieve token embeddings during self-attention: rather than recomputing attention scores for every token at every step, transformers store keys and values for previously seen tokens. In MLMs, this is operationalized by storing pre-computed visual information as static key-value tokens in the cache, allowing text tokens to selectively retrieve them via causal cross-modal attention.  

\noindent \textbf{Causal attention.} In autoregressive decoding, a causal mask $M$ is applied, preventing tokens from attending to future positions:
\[\text{Attention}(Q, K, V) = \text{softmax}\left(\frac{Q(K)^T}{\sqrt{d_k}} + M\right) V\]
% Here, the mask $M$ ensures that each token can only attend to previous tokens and itself. 
In MLMs, the image is generally positioned before the text in the input. Hence, causal attention ensures that text tokens only attend to previous text and visual tokens, and that visual tokens do not attend to text tokens (i.e., there is one-way querying), allowing them to be pre-computed and stored statically in the KV cache (c.f. Appendix \ref{sec:gqa} for details). 

\noindent \textbf{Cross-modal attention.} Due to the positioning of images before text in the input, the LLM can query visual features when generating text via causal attention, i.e., they can ``look up'' relevant visual information:
$\text{Attention}(Q_\text{text}, K_\text{vision}, V_\text{vision})$.
Vision tokens do not influence text generation directly, i.e., they do not modify the text keys or values (similar to how a text token does not modify successive text tokens in the input).

\noindent \textbf{Text generation by the language  model.} The weighted sum of values omitted by the attention mechanism is passed through the remainder of the transformer block to the next layer, successively until the final layer, when it is normalized, passed through a linear layer and softmax, and generates a prediction probability distribution over the vocabulary, predicting each token of the output auto-regressively. 

% Why we care about values in our probing tasks. 

%In our work, to understand the visual representations within the language model, we study the keys and values in the attention mechanisms corresponding to the image input (c.f. Figure \ref{fig:teaser}). 
%This is for two reasons: firstly, due to the positioning of the image before the text and the use of causal attention, the image keys and values are not influenced by the text input, and serve as a \textbf{purely visual representation};
%and secondly, the visual key-value pairs, once computed, are stored and fixed, allowing text tokens to attend to the keys and retrieve values that \textbf{directly contribute to the output}. Thus, they act as a \textit{proxy for the input image}, remaining accessible throughout any downstream language task.
%Therefore, if we desire stronger perception capabilities from our models, studying what is encoded by the image KVs in the language model is a necessary step.

To understand visual representations within the language model, we study the image-based keys and values in the attention mechanism (c.f. Figure~\ref{fig:teaser}). First, due to causal attention and the typical position of image before text, these key-value pairs are unaffected by the text input and thus form a \textbf{purely visual representation}. Second, once computed, they are stored and fixed, allowing all text tokens to attend to image keys and retrieve values that \textbf{directly contribute to the output}. As such, they serve as a \textit{proxy for the input image}, remaining accessible throughout any downstream language task. Understanding what is encoded in these representations is therefore essential for improving perception in MLLMs.



==> sections_v1/4_flow.tex <==
\section{Flow of Visual Information through the Language Model}
\label{sec:flow}
% How LLM layers process (improve-then-degrade) visual information (segmentation+correspondence numbers) 
Despite the use of strong vision encoders such as SigLIP \citep{zhai2023sigmoid}, VLMs
continue to perform poorly on vision-centric benchmarks \citep{fu2024blink, tong2024eyes}. This suggests that the language model may not be processing visual information passed into it by the vision encoder correctly. 
We study the flow of visual information through the language model by probing the image \textit{value} tokens in the KV cache of each layer of the language model.

% on perception-heavy tasks such as segmentation and correspondence.


\noindent \textbf{Why values?} As discussed in Section \ref{sec:preliminary_llm}, image value tokens serve as a proxy for the input image at each layer within the language model. Further, individual image values contribute to MLM language generation by aggregating spatially distributed information, per the position encoding added to the corresponding image key. 
Therefore, image values should \textit{encode well-localized semantics} of the image while \textit{maintaining cross-modal alignment}. 

\noindent \textbf{Probing tasks.} To assess whether image values contain the aforementioned visual information, we probe them on two types of tasks requiring the same: segmentation and correspondence. We discuss each task alongside its experimental setup in greater detail below. Note that all tasks are performed in a \textbf{zero-shot} manner unless otherwise specified.

\noindent\textit{Few-shot foreground segmentation.} We evaluate on Pascal-5i (split 0) \citep{shaban2017one}. We train a linear classifier on top of each image value to perform 5-shot binary segmentation. 

\noindent\textit{Co-segmentation.} We evaluate on MSRC \citep{shotton2006textonboost}, which contains sets of images across which the model must segment a similar object. For each image value, we follow \cite{amir2021deep} and perform spatial clustering to segment objects across images.

\noindent\textit{Semantic segmentation.} We evaluate on ImageNet-S \citep{gao2022luss}. We project the text of the class name into the representational space of the image values using the MLM (independent of the image), then choose the final text token as the representation of the class. We select image values with highest dot product with this text token as the segmented region.

\noindent\textit{Referring expression segmentation.} We evaluate on RefCOCO \citep{kazemzadeh2014referitgame}, which requires grounding language to an object in the image. We follow the same method as semantic segmentation, but with text of the referring expression rather than class name. 

\noindent\textit{Semantic correspondence.} We evaluate on SPair71K \citep{min2019spair}, in which models must establish semantic correspondences between keypoints annotated on pairs of images. We find nearest neighbors between images for each image value corresponding to a keypoint.

\noindent\textit{Temporal correspondence.} We evaluate on DAVIS \citep{pont2017davis}, in which models track keypoints of an object across video frames. We follow the same method as for semantic correspondence.


% \begin{enumerate}
%     \item \textit{Few-shot foreground segmentation.} We evaluate on Pascal-5i (split 0) \citep{shaban2017one}. We train a linear classifier on top of each image value to perform 5-shot binary segmentation. 
%     \item \textit{Co-segmentation.} We evaluate on MSRC \citep{shotton2006textonboost}, which contains sets of images across which the model must segment a similar object. For each image value, we follow \cite{amir2021deep} and perform spatial clustering to segment objects across images.
%     \item \textit{Semantic segmentation.} We evaluate on ImageNet-S \citep{gao2022luss}. We project the text of the class name into the representational space of the image values using the MLM (independent of the image), then choose the final text token as the representation of the class. We select image values with highest dot product with this text token as the segmented region.
%     \item \textit{Referring expression segmentation.} We evaluate on RefCOCO \citep{kazemzadeh2014referitgame}, which requires grounding language to an object in the image. We follow the same method as semantic segmentation, but with text of the referring expression rather than class name. 
%     \item \textit{Semantic correspondence.} We evaluate on SPair71K \citep{min2019spair}, in which models must establish semantic correspondences between keypoints annotated on pairs of images. We find nearest neighbors between images for each image value corresponding to a keypoint.
%     \item \textit{Temporal correspondence.} We evaluate on DAVIS \citep{pont2017davis}, in which models track keypoints of an object across video frames. We follow the same method as for semantic correspondence.
% \end{enumerate}

\input{tables/segmentation_correspondence}

\begin{figure*}[]
    \centering
    \includegraphics[width=\textwidth]{figures/layer_seg_corr_fig.pdf}
    \caption{Average segmentation across 4 tasks for LLaVA-OneVision 7B. (top left) Maximum-per-layer performance. (bottom left) Performance per head. Performance peaks at layer 15. c.f. Appendix for per-task information. \amita{TODO:  Discuss correspondence} 
    % \ranjay{Rename titles of graphs to "Segmentation (or Correspondence) performance across layers from value tokens "} 
    % \ranjay{What is going on in the heatmap? There are weird red fonts and legend is hidden. Is it showing the same thing?}
    }
    \label{fig:layer_seg}
\end{figure*}

\noindent\textbf{Best value results.} \ranjay{Paragraph is very confusing. The term "best value" is confusing. Can we use something better?}
We report the highest performance across all values, i.e., across all heads and layers in the model, as ``best value'' performance. 
As seen in Table \ref{tab:segmentation_correspondence}, MLM visual representations show the capability to perform a wide variety of perception tasks, from different types of segmentation to different types of correspondence across images. 

\noindent\textbf{Comparison to input visual representations.}
We compare the best value results to the performance of the input visual representation to the language model, i.e., the representation produced by the projection layer after the visual encoder. 
The best value outperforms the input visual representation in all six tasks of segmentation and correspondence. 
This shows that the language model does perform processing of the visual information it receives, adding to the information contained by the visual representations. \ranjay{Weird sentence structure. Also the main takeaways are all hidden away somewhere in the paragraphs and the bolded part is unhelpful. Can we just change the bolded sentences to be the main takeaway?} 

% This suggests that some heads in the language decoder have developed a significantly better understanding of shape than either the visual encoder or the projector output. It implies that the language decoder, after multimodal finetuning, has evolved beyond being a purely language model.

\noindent\textbf{Flow through the model.} Having shown that the language model does add \ranjay{I find the term "add" to be not the right one. Perhaps "refine"? Can we change it to that everywhere, including the abstract?} to the visual information contained in the input visual representation, we now study how that process evolves across the layers of the language model. 
% We evaluate performance of each value, i.e. the value corresponding to each head in each layer through the model. 
% We compare these to the input visual information, i.e., the performance of the post-projection SigLIP visual representation. This tells us how the layers treat the visual information.
Figure \ref{fig:layer_seg} (bottom) depicts the average segmentation and correspondence performance of the value tokens corresponding to  each head in each layer of the language model. 
Figure \ref{fig:layer_seg} (top) tracks the maximum performance per layer. 
The early layers (1--15) slowly build upon the visual information contained by the visual representations. 
This information peaks at layers 14--15, after which it falls off steeply across the later layers of the model, as the model begins to focus on generating a text output. 
This is similar to the processing of semantic information by language models \citep{Tenney2019BERTRT}. c.f. Appendix for per-task observations. 
% \amita{Put per-task observations here, and figures in the appendix.}

\noindent\textbf{Comparison to SigLIP.} LLaVA-OneVision 7B uses the SigLIP v1-384 model as its visual encoder. 
However, it finetunes the visual encoder during training. We compare the performance of the visual encoder of LLaVA-OneVision 7B (post-projection) with the original SigLIP v1-384 model in Table \ref{tab:segmentation_correspondence} (bottom) across all 6 tasks \ranjay{This is the first time "6 tasks" is used in this section.}. \ranjay{It is not obvious at all what the third row is when reading the table. Calling it SigLip is misleading.}
We find that across all 6 tasks, SigLIP outperforms its LLaVA-finetuned version. \ranjay{Ok, now I am not sure I even know what you are referring to. I have no idea how to connect the text to the rows in the Table. Can you make the naming consistent and the messaging clearer?}
While not optimal, this is perhaps not too surprising, as the finetuning focuses on multimodal tasks over pure perception tasks.
More interesting, though, is that in 3 of 6 tasks \ranjay{Maybe mention which tasks? Or at least highlight it in the table for easy reading?}, SigLIP outperforms the best value across the language model---hinting that the language model is not able to compensate for the lost information. We will discuss in Section \ref{sec:intermediate_vs_vqa} how this impacts the text output of the model, but this agrees with observations from \citet{fu2025hidden} that VLMs underperform visual encoders.

\noindent\textbf{Comparison to other visual encoders.} 
In Table \ref{tab:visual_encoders_correspondence}, we compare the best value performance of LLaVA-OneVision 7B to that of CLIP \citep{RadfordKHRGASAM21} and DINO \citep{caron2021emerging} visual representations on semantic and temporal correspondence tasks. 
We find that the best value outperforms both CLIP and DINO on semantic correspondence, and that it outperforms CLIP on temporal correspondence (but not DINO). 
This can be partially attributed to the benefits of cross-modality of the value tokens, and partially attributed to the training procedure of LLaVA-OneVision, which includes multi-image and video data---similar to the pairs of images in correspondence tasks.

\input{tables/combined_correlation_correspondence}

\noindent\textbf{Results of other models.} We run these experiments across two other VLMs: LLaMA-3-LLaVA-NeXT 8B \citep{li2025llavanextinterleave} and Qwen2.5-VL 7B \citep{bai2025qwen25vltechnicalreport}. \textcolor{red}{Observations}. c.f. Appendix for complete results and figures. \ranjay{Say that the results are consistent.}

\ranjay{This section had a bunch of conclusions that are all hidden away throughout the section. Can we either make them obvious or add a summary at the end? I don't even remember what was better than what by the end of reading. The tables and figures don't help either.}

==> sections_v1/5_visual_representations.tex <==
\section{Better Visual Representations in the Language Model}
\label{sec:better_visual_representations}
Thus far, we have discussed how language model layers process visual information, studying the quality of visual representations in the language model.
This raises two questions: (1) Do we actually need high-quality visual representations? \ranjay{of course we do? Is this even a real research question?} and (2) If so, how do we obtain them? \ranjay{By making better visual encoders? I don't get these questions. Questions usually have multiple potential answers. Doesn't seem like these do.}


\ranjay{Ok coming back after reading section 5.1, the real question you are asking is "do we actually need high-quality visual representations \textit{inside the LLM}? This is not clear at all. Also, I am still not sure why this is worth asking unless you are going to show that Mahtab's model (or another model), which should retain more visual information also has better end-to-end performance.}

In Section \ref{sec:values-correlate}, we address the first question: we study the impact of visual representation quality on overall VLM performance, finding that better perception of visual representations correlates with better perception of the VLM. 
In Section \ref{sec:prefixing}, we begin \ranjay{only begin? Do you continue? If not, then just ask the part of the question you do answer.} to address the second question: we present preliminary experiments that highlight the use of textual prefixing to improve visual representation quality, and discuss the need for future research to improve them further.


\subsection{Better perception of image values correlates with better perception of the model}
\label{sec:values-correlate}
% There's a correlation between better visual representations and better perception of the model, so we need better visual representations
Having studied the perception capabilities of MLMs' intermediate \ranjay{You don't usually call it "intermediate representations" in other parts of the paper.} \ranjay{nevermind, i think you bring it up in the context of section 6.} representations by probing image value tokens for the perception-heavy tasks segmentation and correspondence, we now assess MLMs' end-to-end perception reasoning by evaluating them on the perception-heavy vision-language reasoning tasks in CV-Bench \citep{tong2024cambrian} and BLINK \citep{fu2024blink}. 
This allows us to investigate a key question: \textit{Does improved perception of intermediate visual representations correlate with better perception reasoning of the model itself?} If so, this would motivate the need to further study visual representations within the language model.
% motivates further study of intermediate representations

\noindent \textbf{Experiment.} 
% We calculate the perception capabilities of the MLM intermediate visual representations by using the maximum segmentation performance across all image values, averaged across four segmentation benchmarks: Pascal-5i, MSRC, ImageNet-S and RefCOCO (c.f. Section \ref{sec:values-tasks}).
To calculate MLMs' end-to-end perception reasoning capability, we evaluate on two vision-centric VQA benchmarks: CV-Bench, and the perception-heavy tasks in BLINK. 
CV-Bench consists of 2,637 test samples and assesses MLMs' 2D and 3D perception capabilities in a single image, covering four major categories: counting, relations, depth estimation, and distance estimation. BLINK, on the other hand, contains single-image and multi-image questions. Since certain question types in BLINK, such as art style \ranjay{Oh, is this why you bring up art styles in the intro? It's too low level. Let's remove it from the intro.}, are less relevant to perception, we select a subset of BLINK consisting of four perception-related tasks: counting, object localization, relative depth, and spatial relations, totaling 1,021 test samples. We evaluate MLMs across these 3,658 test samples to estimate their perception reasoning ability. We compare this to MLM values' segmentation capabilities averaged across four tasks: Pascal-5i, MSRC, ImageNet-S and RefCOCO (c.f. Section \ref{sec:flow}).

\label{sec:downstream_correlation}

% \begin{wrapfigure}{l}{0.5\textwidth}
% \vspace{-1.5em}
% \includegraphics[width=0.95\linewidth]{figures/segmentation_vs_downstream.pdf} 
% \caption{Segmentation performance of LLAVA-OneVision and QwenVL models versus downstream performance. Segmentation is averaged across four datasets, and downstream performance is averaged across CV-Bench and a subset of BLINK (c.f. Section \ref{sec:downstream_correlation}).} 
% \vspace{-2em}
% \label{fig:downstream_correlation}
% \end{wrapfigure}

We evaluate two MLMs with different configurations: (1) models of the same version but different sizes: LLaVA-OneVision (0.5B, 7B, 72B); and (2) models of the same size but different versions: Qwen2-VL 7B and Qwen2.5-VL 7B.  
The LLaVA-OneVision 0.5B model stores 2 key-value pairs per layer, the 7B model stores 4 key-value pairs per layer, and the 72B model stores 8 key-value pairs per layer.


\noindent \textbf{Results.}  
As shown in Figure \ref{fig:downstream_correlation}, we observe that MLMs of different sizes and versions exhibit the same trend: the stronger the perception capability of their image values, as estimated by their segmentation performance, the better the MLMs themselves perform on downstream perception reasoning vision-language tasks.

This finding shows that improved perception of MLM intermediate visual representations goes hand-in-hand with better perception reasoning capabilities of the model itself on perception-heavy vision-language tasks---showing the importance of high-granularity visual representations, and
further emphasizing the need to study the same in MLMs.

% This finding supports two key conclusions. First, value tokens that better encode well-localized semantics positively contribute to MLMs' performance on vision-language tasks. Second, the challenges in MLMs' end-to-end perception-reasoning partly stem from perception itself—that is, the inability to learn sufficiently good visual representations for downstream language tasks, rather than merely being a vision-language alignment issue.


\subsection{Improving visual representations by leveraging their cross-modal and promptable nature}
% in the LM?
\label{sec:prefixing}
Having established the need to improve the perception capabilities of visual representations within the language model, we now investigate one possible method to accomplish the same: \textit{textual prefixing}.

% Preliminary experiments show you can improve visual information in values with prefixing, but we need more research to improve them further

Visual representations in the language model have an interesting capability thanks to their cross-modal nature: 
% Being cross-modal, visual representations in the language model have an advantageous capability: 
they can be made \textit{promptable} by prefixing textual prompts to the visual input. This flexibility allows the model to dynamically adapt its visual representations to better align with specific tasks, in a zero-shot manner.
We study this in the context of three tasks: referring expression segmentation, semantic correspondence, and domain adaptation for semantic segmentation. We discuss the results shown in Table \ref{tab:prefixing_results}.
% one segmentation task from the previous experiments (referring expression segmentation), one correspondence task from the previous experiments (semantic correspondence), and an additional task particularly suited to testing promptability (domain adaptation for semantic segmentation).

% We study this in the context of three tasks: referring expression segmentation, semantic correspondence, and domain adaptation for semantic segmentation.


\input{tables/prefixing}

\noindent\textbf{Referring expression segmentation.}
We evaluate image values from LLAVA-OneVision 7B on RefCOCO. Without text prefixing, the experiment is as described in Section \ref{sec:flow}. When a textual prefix is added to the image input (here, the image caption sourced from COCO captions \citep{chen2015microsoftcococaptionsdata}),
% the image caption sourced from COCO captions \citep{chen2015microsoftcococaptionsdata} is prefixed to the image input, 
the image values achieve modestly improved segmentation results. This shows that the visual representations were able to incorporate the text caption---which contains information about the image, and may contain information about the object to segment---to improve their textual grounding and segmentation capabilities.

\noindent\textbf{Semantic correspondence.} We evaluate image values from LLAVA-OneVision 7B on SPair71K. Without text prefixing, the experiment is as described in Section \ref{sec:flow}. The textual prefix we add here is the class name of the object in the image. As with referring expression segmentation, the semantic correspondence performance improves slightly with prefixing, showing that the visual representations incorporate textual information from the prefix to improve textual grounding and segmentation capabilities. 


\noindent\textbf{Domain adaptation for zero-shot semantic segmentation.} 
We evaluate image values from LLAVA-OneVision 7B on BDD-100K \citep{yu2020bdd100k} on two domains: city street during daytime, and highway during nighttime. By prefixing the image with text specifying the domain (``The image is taken at \{daytime, nighttime\} and it is from \{city street view, highway\}''), performance improves on both domains, but more significantly on the more challenging one. This shows that the visual representations successfully incorporate the text information identifying the domains, then adapt to each.

\noindent\textbf{Controls.} We run two controls for this experiment, to ensure the \textit{content} of the text prefix was what improved the visual representation quality, not the addition of a text prefix itself. For all tasks, we prefix a random string of text (``A rustic wooden table filled with freshly baked croissants, dripping honey, and a steaming pot of Earl Grey tea beside a bowl of ripe figs.'') to the image and calculate performance (``Prefixing-random''). Across all tasks, this does not improve performance compared to no prefixing, and rather lowers it slightly. For the semantic correspondence task, we add a second control wherein we prefix the name of the \textit{incorrect} class (``Prefixing-incorrect''). We do the same for domain adaptation, in which we prefix the name of the \textit{incorrect} domain (``The image is taken at daytime and it is from city street view'' for an image of night+highway, and vice versa). These numbers are even lower than the random prefix for both tasks. These results collectively show that it is indeed the prefix content that improves visual representation quality.

Our findings suggest that image values are not only effective for visual understanding, but are also inherently adaptable to linguistic conditioning.
% , enabling more controllable reasoning in both pure-vision (semantic segmentation) and vision-language (textual grounding) tasks.
Further, they set forth a promising method to improve perception capabilities of image value tokens, which we have seen in Section \ref{sec:values-correlate} correlates with overall VLM perception capability. However, there remains room for improvement, calling for further research in improving quality of visual representations within the language model.

==> sections_v1/6_text_output.tex <==
\section{Better Language Model Utilization of Existing Visual Representations}
% if we really do this...
% Alt title: "better LM output with existing vis rep"
\label{sec:better_output}
Having highlighted the need for better visual representations within the language model, as well as a method to improve them, we now discuss improvement of the text output of the overall VLM by better leveraging the \textit{existing} visual representations. We tackle this in two parts: in Section \ref{sec:intermediate_vs_vqa}, we show that visual representations are not currently being leveraged by VLMs to their fullest; and in Section \ref{sec:keys}, we reveal a contributing factor to this behavior via an intervention study, calling for further research.
% intervene on visual representations to improve VLM performance on two benchmarks.

\subsection{Language Models under-utilize the visual information in their visual representations}
\label{sec:intermediate_vs_vqa}
While better visual representations are needed, and correlate with overall model perception capabilities (Section \ref{sec:values-correlate}), it is unclear how much of the perception capabilities of the intermediate visual representations are utilized by the model. To put this case in point, we have shown in Sections \ref{sec:flow} and \ref{sec:better_visual_representations} that VLM visual representations are capable of perception-heavy tasks---but our motivation to study them was rooted in the poor performance of VLMs on end-to-end perception reasoning \citep{fu2024blink, tong2024eyes}. This hints that VLMs are not optimally leveraging their existing visual representations.

% Even within the visual representations we have, best performance doesn’t reach the text output (intermediate-vs-VQA) --- we need to better leverage our visual representations to improve text output

% Our motivation to study the intermediate visual representations of MLMs was their poor performance on end-to-end perception reasoning \citep{fu2024blink, tong2024eyes}. How, then, are their image values capable of perception, as we show in Sections \ref{sec:values-tasks}--\ref{sec:values-clip}? 
% We find that, although the visual representations may be capable of perception, this capability does not always propagate through the model to the text output: revealing room for improvement to surface the capabilities already present within MLMs.

\noindent\textbf{Experiment.} Perception-heavy tasks can be framed as VQA; they can also be evaluated directly from the visual representations (as in Section \ref{sec:flow}).
We posit that the image values \ranjay{you mean value tokens?} being able to perform a task on an example is a sufficient 
(if not necessary, in case the language model can compensate with its reasoning capabilities) 
condition for the MLM answering the VQA corresponding to the example correctly.
We perform this evaluation on four tasks: semantic correspondence, multi-view reasoning, art style and visual similarity.
% We first frame semantic correspondence in SPair71K as a VQA task, as in BLINK (for which image coordinates are not public), generating 200 samples. We evaluate the MLM on VQA. We then evaluate its intermediate values on semantic correspondence as an image pair, as in Section \ref{sec:flow}. 
% \footnote{As we did not have the image coordinates for semantic correspondence on BLINK, we recreate the VQA task with SPair71K images, following the same method as BLINK (itself sourced from SPair71K).} 
We calculate the fraction of instances where the MLM predicts the VQA answer incorrectly, \textit{despite its image values predicting correctly for the same input}. 

\noindent\textbf{Results.} \ranjay{I think a cardinal rule of paper writing is being violated in this paper everywhere. I can't find any mention of what VLM and what VR means or what their union means in Table 4. Your text should match your tables. I have no idea what this section experiments are even doing to be honest. Also, i have no idea what intermediate tokens you are using. I have no idea how you actually use the intermediate ones to make predictions, etc.} As shown in Table \ref{tab:intermediate_vs_vqa}, language models under-utilize visual information present in the model on all four tasks. In the case of art style, this is particularly egregious, with performance increasing by 33.3\% if the model had successfully surfaced the perception capability of its visual representations. Across all tasks, the percentage of instances where the intermediate value was incorrect but the MLM prediction was correct is very low, showing the importance of visual representations for these tasks.

% The accuracy of LLAVA-OneVision 7B on semantic correspondence VQA is 36\%. On only 2.5\% of these, the intermediate value was incorrect but the MLM prediction was correct, showing the importance of visual representations for this task. However, on 7.5\% of the examples, the MLM predicted incorrectly despite the intermediate values predicting correctly! In other words, if the model had successfully surfaced the perception capability of its visual representations, it would have achieved an accuracy of 43.5\% rather than 36\%. c.f. Table \ref{tab:intermediate_vs_vqa}. \textcolor{red}{Update with multi-view, art style, visual similarity results.}

% value yes, MLLM yes: 67 --> 33.5
% Only value correct (value yes, MLLM no) : 15 --> 7.5
% Only MLLM correct (value no, MLLM yes) : 5 --> 2.5
% Both incorrect (value no, MLLM no) : 113 --> 56.5

% Our finding reconciles the perception capabilities of MLMs' intermediate visual representations with their subpar performance on perception reasoning tasks. More importantly, it reveals the potential of MLMs to achieve better perception: underscoring the need for future work to focus on surfacing the capabilities already present within MLMs.

Our finding reveals that language models currently under-utilize the visual information in their intermediate visual representations. 
% Cite Berkeley? I don't actually know what it says
This reconciles the perception capabilities of MLMs' intermediate visual representations with their subpar performance on perception reasoning tasks---but more importantly, it reveals the potential of MLMs to achieve better perception: underscoring the need for future work to focus on surfacing the capabilities already present within MLMs.

\input{tables/combined_intermediate_intervention}


\subsection{Intervening on visual representations can improve Language Model output}
\label{sec:keys}
% There are also other ways to leverage visual representations to improve text output: by intervening on keys.

% Having revealed that visual representations contain more information than is captured by the language model text output, we conduct an intervention to identify 

Having revealed that there are instances wherein sufficient visual information was present in the intermediate visual representation, but was not captured by the language model in its text output, we now study a potential reason why this could occur. 

\citet{darcet2024vision} reveal that in ViTs, tokens in middle layers corresponding to background patches tend to encode input-agnostic artifacts rather than useful information about the image.
% , since these regions lack meaningful content. 
We investigate whether a similar phenomenon occurs in language models processing visual information, by identifying input-agnostic visual representations in the language model. 
If input-agnostic visual representations in later layers of the langauge model do encode artifacts, it would partly explain why VLMs are under-utilizing the visual information in their visual representations: because they are distracted by these artifacts.

\noindent \textbf{Identifying input-agnostic keys.}
We randomly sample 1000 images from MSCOCO \citep{lin2014microsoft} and obtain intermediate visual representations for each sample from LLaVA-OneVision 7B. 
We compute the variance of image key tokens in each head and layer across the samples. 
We find that the variance forms a bimodal distribution, which we split with a threshold to define input-agnostic keys
% We find that the variance forms a bimodal distribution, with the first mode centered at a variance of 200, and the second at 600. 
% Setting a threshold at the lowest point between these two modes at a variance of 450, 
% we refer to keys with variance below this threshold as input-independent keys, and those above as input-dependent keys. 
(details in Appendix).

% As shown in Figure \ref{fig:key_visualization}, we find that when setting this threshold: (1) 20 keys are input-independent in the first 8 layers, including all 16 keys in the first 4 layers; (2) 8 keys are input-independent in the next 10 layers; and (3) 14 keys are input-independent in the last 10 layers.
% We call these the early layers, middle layers and late layers respectively.

As shown in Figure \ref{fig:key_visualization}, we find that when setting this threshold, input-agnostic keys dominate in earlier layers of the language model, but, critically, re-emerge in later layers. We test whether these input-agnostic keys in later layers too, contain input-agnostic artifacts as in ViTs with an intervention study.
% with the POPE benchmark \citep{li-etal-2023-evaluating} and four subsets of the MME benchmark \citep{fu2023mme} which together address hallucination and general perception capabilities (c.f. Appendix).

% Following the setup from "Self-Correcting Decoding with Generative Feedback for Mitigating Hallucinations in Large Vision-Language Models" (Zhang et al, ICLR 2025), we evaluate on these subsets of MME: count, color, position and existence. In all four of these, the model is asked a Yes/No question about the image (similar to POPE), which address hallucination across various axes and also measure general capabilities (addressing R3's concern).

% Our analysis reveals that key tokens can be categorized into two distinct types based on their variance:  
% (1) \textit{Input-independent keys.} These keys have very low (L2$<$200) variance across the input images. 
% Most keys in early layers of MLMs are input-independent, and a smaller number of input-independent keys reappear in middle-to-late layers of the language model. 
% % typically emerge in earlier layers of the model, although there are some input-independent keys in later layers as well. 
% (2) \textit{Input-dependent keys.} These keys have a much higher variance across the input images. They typically dominate in the middle-to-late layers of the model. 

% We visualize all image keys of LLaVA-OneVision 7B for two images with a PCA projection in Figure \ref{fig:key_visualization}. Although the two images are very different, the input-independent keys can be seen to remain near-invariant (c.f. Appendix \ref{sec:key_visualization_section} for more visualizations across models).

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/key_visualization.pdf}
    \caption{PCA visualization of all image keys in LLaVA-OneVision 7B for two COCO images. The input-independent image keys (highlighted) alone are nearly constant across images.}
    \label{fig:key_visualization}
    \vspace{-0.5cm}
\end{figure*}

% Blocking values corresponding to input-independent keys
\noindent\textbf{Intervening on input-agnostic key-value pairs.} 
We conduct an interventional study, blocking text token queries to input-agnostic image keys in later layers via attention knockout \citep{geva2023dissecting}. 
Notably, we do \textit{not} block text keys that belong to the same attention head as these input-agnostic image keys, ensuring a focus on understanding the impact of visual representations on model output.
We evaluate on two benchmarks: POPE \citep{li-etal-2023-evaluating}, and 4 subsets of MME \citep{fu2023mme} which together address hallucination and general perception capabilities. 
As shown in Table \ref{tab:intervention}, we find that blocking image-agnostic keys (and thus, values) in later layers improves model performance on both benchmarks.

We posit that input-agnostic image keys in earlier layers play an essential role in aggregating contextual information consistent across different inputs, whereas middle-to-later layers of the model gradually shift focus toward understanding semantics \citep{neo2024towards}, similar to CNNs \citep{krizhevsky2012imagenet} and pure-text language models \citep{Tenney2019BERTRT}, thus have fewer input-agnostic visual representations. 
Hence, the input-agnostic image keys in later layers of the model are likely to encode artifacts, similar to ViTs \citep{darcet2024vision}.  
By removing the influence of these visual representations on the language output, we successfully improve the output of the VLM.

Our intervention experiment sheds light on a potential reason for VLM under-utilization of visual information encoded by the visual representations within the language model.
While our results highlight a method to improve language model utilization of existing visual representations, further research is needed to solve the problem at its root, i.e., to improve the overall quality of visual representations within the language model to in turn improve the performance of the VLM itself.


% We conduct experiments with LLaVA-OneVision 7B on the POPE benchmark \citep{li-etal-2023-evaluating}, a dataset with 9,000 test samples designed to evaluate MLM hallucination via object identification. Each question in the benchmark asks whether a specific object exists in the given image. We report F1 score aggregated across all 3 subsets of the benchmark.
%on all three subsets of the benchmark: random, popular and adversarial.

% All image keys in the first four layers of LLaVA-OneVision 7B are input-independent. A smaller number of input-independent keys reappear in the last ten layers. 

% Input-independent image keys occur often in early layers, with all keys in the first four layers being input-independent. A smaller number reappears in the last ten layers. 
% We conduct an interventional study, blocking text token queries to input-independent image keys in: (1) the first four layers of the model; then (2) the last ten layers of the model.
% This method is referred to as ``Attention Knockout'' \citep{geva2023dissecting}.
% Notably, we do \textit{not} block text keys that belong to the same attention head as these input-independent image keys, ensuring a focus on understanding the impact of visual representations on model output.

% \noindent \textbf{Results.}  
% LLaVA-OneVision 7B achieves an F1 score of \textbf{78.1} on POPE. When we intervene on attention to the input-independent keys in the first four layers of the model, performance drops sharply to an F1 score of \textbf{55.4}. However, when we intervene on attention to the input-independent keys in the last ten layers of the model, performance increases to an F1 score of \textbf{81.3}, scoring higher (i.e., hallucinating less) than the original model.



==> sections_v1/7_discussion.tex <==
\section{Discussion and Future Work}
\label{sec:discussion}
Our investigation throws light on an as-yet under-explored component of MLMs: the visual representations stored in the key-value cache and attended to during text generation, in contrast to existing work, which has studied the transformer block outputs within MLMs \citep{neo2024towards, zhang2024large}.
We find that: (1) language models build upon the visual token information in earlier layers, then lose it in later layers, with the highest performance being less than that of SigLIP on 3 of 6 tasks we study; (2) better perception of image value tokens correlates with better perception of the VLM on downstream tasks, and can be improved via textual prefixing; (3) language models under-utilize the visual information in their existing visual representations, partly because later input-agnostic representations encode artifacts, which in turn can be intervened on to improve the language model output. 
% We find that: (1) a deeper understanding of what these tokens encode allows us to make interventions to improve the model; (2) image value tokens can perform perception tasks, and their performance goes hand-in-hand with perception reasoning of the MLM itself; (3) cross-modality of the visual representations allows benefits such as promptability for flexible task adaptation, as well as outperforming pure-visual representations even on pure-vision tasks; and (4) the perception capabilities of image value tokens reveal room for improvement in perception reasoning by MLMs.
% , calling for research in surfacing these intermediate visual representations' capabilities in the output of the model itself. 

Our work calls for research in three main directions: first, improving finetuning of visual encoders like SigLIP in multimodal training so the projected visual information provided to the language model is not inferior to that of the original visual encoder; second, improvement of visual representations within the language model by leveraging traditional text-only methods such as prompting; third, improving language model utilization of existing visual information, potentially by preventing the occurrence of artifacts in later language model layers. 
% Our work calls for research in three main directions: first, studying more closely what text is generated when various image keys are attended to or blocked to determine whether fixed image keys have fixed purposes (as suggested by Section \ref{sec:keys}); second, understanding more deeply the benefits of cross-modality on vision and vision-language tasks; and third, surfacing intermediate visual representations' perception capabilities in the output of the model itself.
Our work highlights the importance of interpreting image processing by MLMs by studying visual representations in language models, and shows promise for the future of perception reasoning in MLMs.

==> tables/combined_keys.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{0.55\textwidth}
    % \footnotesize
    % \begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/key_vis.pdf}
    \caption{PCA visualization of all image keys in LLaVA-OneVision 7B for two COCO images. The input-agnostic image keys (highlighted) alone are nearly constant across images.}
    \label{fig:key_visualization}
    % \vspace{-1em}
% \end{figure}
    \end{minipage}
    \hspace{0.01\textwidth}
    \begin{minipage}{0.4\textwidth}
    \footnotesize
    \centering
        \addtolength{\tabcolsep}{-0.3em}
        \begin{tabular}{lcc}
        \toprule
            Model& POPE & MME*\\
            \midrule
            LLaVA-OneVision 7B & 78.1 & 173.3\\ 
            % Intervention-early & 65.1 & -  \\
            % Intervention-mid & 77.9 & -  \\
            + intervention & \textbf{81.2} & \textbf{179.0}  \\
          \bottomrule 
        \end{tabular}
    \captionof{table}{
    Our intervention reveals image keys that contain artifacts, as blocking them improves MLM performance on POPE and MME.
    % Our intervention on the visual representations improves model performance on POPE and a *subset of MME.
    }
    \label{tab:intervention}
    \end{minipage}
    \vspace{-1em}
\end{figure}



% Feature 3 Performance
% val accuracy: 60.9% → this is feature, not VQA. VQA is 45.86%.
% VQA Right Feature Right: 23 → 17.29%
% VQA Right Feature Wrong: 38 → 28.57%
% VQA Wrong Feature Right: 58 → 43.61%
% VQA Wrong Feature Wrong: 14 → 10.53%
% Total: 133 

